Demystifying SGD with Doubly Stochastic Gradients

Optimization objectives in the form of a sum of intractable expectations are rising in importance (e.g., diffusion models, variational autoencoders, and many more), a setting also known as "finite sum with infinite data." For these problems, a popular strategy is to employ SGD with doubly stochastic gradients (doubly SGD): the expectations are estimated using the gradient estimator of each component, while the sum is estimated by subsampling over these estimators. Despite its popularity, little is known about the convergence properties of doubly SGD, except under strong assumptions such as bounded variance. In this work, we establish the convergence of doubly SGD with independent minibatching and random reshuffling under general conditions, which encompasses dependent component gradient estimators. In particular, for dependent estimators, our analysis allows fined-grained analysis of the effect correlations. As a result, under a per-iteration computational budget of $b \times m$, where $b$ is the minibatch size and $m$ is the number of Monte Carlo samples, our analysis suggests where one should invest most of the budget in general. Furthermore, we prove that random reshuffling (RR) improves the complexity dependence on the subsampling noise.

==> figures/group_isoquad_variance_high_hetero.tex <==

\nextgroupplot[
    xlabel = \(b\),
    ymax   = 30.0,
    ymin   = 0.0,
    xmin   = 1,
    xmax   = 1024,
    legend style={draw=none},
]

	\addplot[color=cherry6, very thick] coordinates {
(1,30.147272115325254)
(2,15.060473484965039)
(4,7.518030123244589)
(8,3.7487203493036843)
(16,1.867889276171868)
(32,0.9351213672832336)
(64,0.48403266819346363)
(128,0.2890788293576732)
(256,0.25278293135796714)
(512,0.3569970251944924)
(1024,0.6538281577855116)
    };
    
	\addplot[color=cherry4, very thick] coordinates {
(1,30.16034740341079)
(2,15.07800988919565)
(4,7.544488759765353)
(8,3.7930234504047533)
(16,1.9478813064335474)
(32,1.0864912558661337)
(64,0.7781582734188051)
(128,0.8687158678678972)
    };
    
	\addplot[color=cherry2, very thick] coordinates {
(1,30.264949708095067)
(2,15.21830112304054)
(4,7.756157851931464)
(8,4.147448259213306)
(16,2.5878175485269823)
    };


==> figures/group_isoquad_variance_low_hetero.tex <==

\nextgroupplot[
    % tuftelike,
    y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=2,
        /tikz/.cd
    },
    %
    xlabel = \(b\),
    ylabel = {Variance},
    ymax   = 2.0,
    ymin   = 0.0,
    xmin   = 1,
    xmax   = 1024,
    legend style={
        draw=none,
        anchor=north east,
        at={(1.05,1.05)},
    },
    legend cell align=left,
]
	\addplot[color=cherry6, very thick] coordinates {
(1,1.8859556618621411)
(2,0.9436282183769147)
(4,0.47342045009396055)
(8,0.24022847287180202)
(16,0.12745629809935952)
(32,0.07871783839041192)
(64,0.06964386389048541)
(128,0.09569738734961672)
(256,0.1699051704973715)
(512,0.32937110490762717)
(1024,0.6538281577855116)
    };
    \addlegendentry{\footnotesize\(mb=16\)}
    
	\addplot[color=cherry4, very thick] coordinates {
(1,1.899030949947676)
(2,0.9611646226075259)
(4,0.4998790866147244)
(8,0.28453157397287104)
(16,0.20744832836103888)
(32,0.23008772697331195)
(64,0.3637694691158268)
(128,0.6753344258598407)
    };
    \addlegendentry{\footnotesize\(mb=128\)}
    
	\addplot[color=cherry2, very thick] coordinates {
(1,2.0036332546319557)
(2,1.1014558564524162)
(4,0.7115481787808353)
(8,0.6389563827814232)
(16,0.8473845704544738)
    };
    \addlegendentry{\footnotesize\(mb=1024\)}


==> figures/group_isoquad_variance_mid_hetero.tex <==

\nextgroupplot[
    xlabel = \(b\),
    ymax   = 6.0,
    ymin   = 0.0,
    xmin   = 1,
    xmax   = 1024,
]
	\addplot[color=cherry6, very thick] coordinates {
(1,7.538218952554764)
(2,3.7669972716945392)
(4,1.8823423847240863)
(8,0.9419268481581784)
(16,0.4755428937138612)
(32,0.24999854416897627)
(64,0.15252162475108105)
(128,0.13437367575122802)
(256,0.18648072266949062)
(512,0.3348962889650002)
(1024,0.6538281577855116)
    };
    % \addlegendentry{\(mb=1024\)}

	\addplot[color=cherry4, very thick] coordinates {
(1,7.551294240640298)
(2,3.7845336759251507)
(4,1.9088010212448503)
(8,0.9862299492592475)
(16,0.5555349239755406)
(32,0.4013684327518763)
(64,0.4466472299764224)
(128,0.714010714261452)
    };
    % \addlegendentry{\(mb=64\)}
    
	\addplot[color=cherry2, very thick] coordinates {
(1,7.655896545324579)
(2,3.9248249097700407)
(4,2.120470113410961)
(8,1.3406547580677997)
(16,1.1954711660689754)
    };
    % \addlegendentry{\(mb=16\)}


==> main-pratendaveragebregman.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateix}\label{thm:prAtEndix}\label {thm:average_bregman} Let \(F : \mathcal {X} \to \mathbb {R}\) be a finite sum of convex functions as \(F = \frac {1}{n}\left (f_1 + \ldots + f_n\right )\), where \(f_i : \mathcal {X} \to \mathbb {R}\). Then, \[ \frac {1}{n} \sum ^n_{i=1} \mathrm {D}_{f_i}\left (\vx , \vx '\right ) = \mathrm {D}_{F}\left (\vx , \vx '\right ), \] for any \(\vx , \vx ' \in \mathcal {X}\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}The result immediately follows from the definition of Bregman divergences as \begin {align*} &\frac {1}{n} \sum ^n_{i=1} \mathrm {D}_{f_i}\left (\vx , \vx '\right ) \\ &\;= \frac {1}{n} \sum ^n_{i=1} \left ( f_i\left (\vx \right ) - f_i\left (\vx '\right ) - \inner {\nabla f_i\left (\vx '\right )}{\vx - \vx '} \right ) \\ &\;= \left (\frac {1}{n} \sum ^n_{i=1} f_i\left (\vx \right ) \right ) - \left (\frac {1}{n} \sum ^n_{i=1} f_i\left (\vx '\right ) \right ) \\ &\qquad - \inner {\frac {1}{n} \sum ^n_{i=1} \nabla f_i\left (\vx '\right )}{\vx - \vx '} \\ &\;= F\left (\vx \right ) - F\left (\vx '\right ) - \inner {\nabla F\left (\vx '\right )}{\vx - \vx '} \\ &\;= \mathrm {D}_{F}\left (\vx , \vx '\right ). \end {align*}\end{proof}


==> main-pratendboundedvariance.tex <==


\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}For any element of the solution set \(\vx _* = \argmin _{\vx \in \mathcal {X}} F\left (\vx \right )\), by \cref {thm:doubly_stochastic_variance}, we have \begin {align*} \mathrm {tr}\V {\rvvg _{\rvB }\left (\vx _*\right )} &\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx _*\right )} \right ) \\ &\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx _*\right )}} \right )}^2 \\ &\qquad + \frac {1}{b_{\mathrm {eff}}} \mathrm {tr}\V {\nabla f_{\rvB }\left (\vx _*\right )}. \shortintertext {Applying \cref {assumption:bounded_variance_both}, we have} &\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \left ( \frac {1}{n} \sum ^n_{i=1} \sigma _{i}^{2} \right ) \\ &\qquad + \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt { \sigma ^2_{i} } \right )}^2 \\ &\qquad + \frac {1}{b_{\mathrm {eff}}} \tau ^2 \\ &= \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) \left ( \frac {1}{n} \sum ^n_{i=1} \sigma _{i}^{2} \right ) \\ &\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum ^n_{i=1} \sigma _{i} \right )}^2 \\ &\qquad + \frac {1}{b_{\mathrm {eff}}} \tau ^2. \end {align*}\end{proof}


==> main-pratenddefaultcategory.tex <==


\prAtEndRestatexi*


==> main-pratenddoublystochasticvariance.tex <==


\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}Starting from the law of total covariance, we have {\setlength {\abovedisplayskip }{1.5ex} \setlength {\abovedisplayshortskip }{1.5ex} \setlength {\belowdisplayskip }{1.5ex} \setlength {\belowdisplayshortskip }{1.5ex} \begin {align} \V {\rvvx _{\rvB }} &= \underbrace { \Esub {\rvB \sim \pi }{ \mathrm {tr}\V { \rvvx _{\rvB } \mid \rvB } } }_{\text {Ensemble Variance}} + \underbrace { \mathrm {tr}\Vsub {\rvB \sim \pi }{ \E { \rvvx _{\rvB } \mid \rvB } }. }_{\text {Subsampling Variance}} \label {eq:doubly_stochastic_variance_main} \end {align} } \par \paragraph {Ensemble Variance} Bounding the variance of each ensemble is key. From \cref {thm:expected_variance_lemma}, we have \begin {align} \E { \mathrm {tr}\V { \rvvx _{\rvB } \mid \rvB } } &= \E { \mathrm {tr}\V { \frac {1}{b} \sum _{i \in \rvB } \rvvx _{i} \,\middle |\, \rvB } } \nonumber \\ &= \E { \mathrm {tr}\V { \sum _{i \in \rvB } \left ( \frac {1}{b} \rvvx _{i} \right ) \,\middle |\, \rvB } } \nonumber \\ &\leq \rho \mathbb {V}{\rvS } + \rho {\left (\mathbb {E}{\rvS }\right )}^2 + \left (1 - \rho \right ) \mathbb {E}{\rvV } , \label {eq:doubly_stochastic_variance_eq1} \end {align} where \begin {align*} \rvS &\triangleq \sum _{i \in \rvB } \sqrt {\mathrm {tr} \V { \frac {1}{b} \rvvx _{i}}} = \frac {1}{b} \sum _{i \in \rvB } \sqrt {\mathrm {tr} \V { \rvvx _{i}}}, \\ \rvV &\triangleq \sum _{i \in \rvB } \mathrm {tr} \V { \frac {1}{b} \rvvx _{i} } = \frac {1}{b^2} \sum _{i \in \rvB } \mathrm {tr} \V { \rvvx _{i} }. \end {align*} In our context, \(\rvS \) is the batch average of the standard deviations, and \(\rvV \) is the batch average of the variance (scaled with a factor of \(1/b\)). \par Notice that \(\rvS \) is an \(b\)-sample average of the standard deviations. Therefore, if \(\pi \) is an unbiased subsampling strategy, we retrieve the population average standard deviation as \begin {align} \Esub {\rvB \sim \pi }{\rvS } = \Esub {\rvB \sim \pi }{ \frac {1}{b} \sum _{i \in \rvB } \sqrt {\mathrm {tr} \V { \rvvx _{i} }} } = \frac {1}{n} \sum _{i = 1}^n \sqrt {\mathrm {tr} \V { \rvvx _{i} }}. \label {eq:doubly_stochastic_variance_eq2} \end {align} Under a similar reasoning, the variance of the standard deviations follows as \begin {align} &\Vsub {\rvB \sim \pi }{\rvS } \nonumber \\ &= \Vsub {\rvB \sim \pi }{ \frac {1}{b} \sum _{i \in \rvB } \sqrt {\mathrm {tr} \V { \rvvx _{i} }} } \nonumber \\ &\;= \frac {1}{b_{\mathrm {eff}}} \Vsub {i \sim \mathrm {Uniform}\left \{1, \ldots , n\right \}}{ \sqrt {\mathrm {tr} \V { \rvvx _{i} }} } \nonumber \\ &\;= \frac {1}{b_{\mathrm {eff}}} \left ( \frac {1}{n} \sum _{i=1}^n \mathrm {tr} \V { \rvvx _{i} } - {\left ( \frac {1}{n} \sum _{i=1}^n \sqrt {\mathrm {tr} \V { \rvvx _{i} }} \right )}^2 \right ), \label {eq:doubly_stochastic_variance_eq3} \end {align} where the last identity is the well-known formula for the variance: \(\mathbb {V}\rvX = \mathbb {E}\rvX ^2 - {(\mathbb {E}\rvX )}^2\). Likewise, the average variance follows as \begin {align} \mathbb {E}_{\rvB \sim \pi } \rvV &= \frac {1}{b^2} \Esub {\rvB \sim \pi }{ \sum _{i \in \rvB } \mathrm {tr} \V { \rvvx _{i} } } \nonumber \\ &= \frac {1}{b} \Esub {\rvB \sim \pi }{ \frac {1}{b} \sum _{i \in \rvB } \mathrm {tr} \V { \rvvx _{i} } } \nonumber \\ &= \frac {1}{b} \left ( \frac {1}{n} \sum _{i=1}^n \mathrm {tr} \V { \rvvx _{i} } \right ) \label {eq:doubly_stochastic_variance_eq4} \end {align} Plugging \cref {eq:doubly_stochastic_variance_eq2,eq:doubly_stochastic_variance_eq3,eq:doubly_stochastic_variance_eq4} into \cref {eq:doubly_stochastic_variance_eq1}, we have \begin {align} &\Esub {\rvB \sim \pi }{ \mathrm {tr}\V { \rvvx _{\rvB } \mid \rvB }} \nonumber \\ &\;\leq \rho \mathbb {V}{\rvS } + \rho {\left (\mathbb {E}{\rvS }\right )}^2 + \left (1 - \rho \right ) \mathbb {E}{\rvV } \nonumber \\ &\;= \frac {\rho }{b_{\mathrm {eff}}} \left ( \frac {1}{n} \sum _{i=1}^n \mathrm {tr} \V { \rvvx _{i} } - {\left ( \frac {1}{n} \sum _{i=1}^n \sqrt {\mathrm {tr} \V { \rvvx _{i} }} \right )}^2 \right ) \nonumber \\ &\quad + \rho {\left ( \frac {1}{n} \sum _{i = 1}^n \sqrt {\mathrm {tr} \V { \rvvx _{i} }} \right )}^2 \nonumber \\ &\quad + \frac {1 - \rho }{b} {\left ( \frac {1}{n} \sum _{i=1}^n \mathrm {tr} \V { \rvvx _{i} } \right )} \nonumber \\ &\;= \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \left ( \frac {1}{n} \sum _{i=1}^n \mathrm {tr} \V { \rvvx _{i} } \right ) \nonumber \\ &\quad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum _{i=1}^n \sqrt {\mathrm {tr} \V { \rvvx _{i} }} \right )}^2. \label {eq:doubly_stochastic_variance_ensemble_variance} \end {align} \par \paragraph {Subsampling Variance} The subsampling noise is straightforward. For this, we will denote the minibatch subsampling estimator of the component means as \[ \bar {\vx }_{\rvB } \triangleq \frac {1}{b} {\sum _{i \in \rvB }} \bar {\vx }_{i}. \] Since each component estimator \(\rvvx _i\) is unbiased, the expectation conditional on the minibatch \(\rvB \) is \begin {align*} \E { \bar {\vx }_{\rvB } \mid \rvB } = \frac {1}{b} {\sum _{i \in \rvB }} \bar {\vx }_{i}. \end {align*} Therefore, \begin {align} \mathrm {tr}\Vsub {\rvB \sim \pi }{ \E { \rvvx _{\rvB } \mid \rvB } } &= \mathrm {tr}\Vsub {\rvB \sim \pi }{ \bar {\vx }_{\rvB } } \nonumber \\ &= \frac {1}{b_{\mathrm {eff}}} \left (\frac {1}{n} {\sum ^n_{i=1}} \norm { \bar {\vx }_{i} - \bar {\vx }}_2^2 \right ). \label {eq:doubly_stochastic_variance_subsampling_variance} \end {align} \par Combining \cref {eq:doubly_stochastic_variance_ensemble_variance,eq:doubly_stochastic_variance_subsampling_variance} into \cref {eq:doubly_stochastic_variance_main} yields the result. Notice that the only inequality we used is \cref {eq:doubly_stochastic_variance_eq1}, \cref {thm:expected_variance_lemma}, in which equality holds if the equality in \cref {assumption:correlation} holds.\end{proof}


==> main-pratendexpectedresidualgradientvariancebound.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateii}\label{thm:prAtEndii}\label {thm:expected_residual_gradient_variance_bound} Let \(F:\mathcal {X} \to \mathbb {R}\) be \(L\)-smooth function. Then, the expected squared norm of a gradient estimator \(\rvvg \) satisfying both \(\mathrm {ER}\left (\mathcal {L}\right )\) and \(\mathrm {BV}\left (\sigma ^2\right )\) is bounded as \[ \mathbb {E} \norm {\rvvg \left (\vx \right )}_2^2 \leq 4 \left (\mathcal {L} + L\right ) \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ) + 2 \sigma ^2, \] for any \(\vx \in \mathcal {X}\) and \(\vx _* \in \argmax _{\vx \in \mathcal {X}} F\left (\vx \right )\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}The proof is a minor modification of Lemma 2.4 by \citet {gower_sgd_2019} and Lemma 3.2 by \citet {gower_sgd_2021}. \par By applying the bound \({(a + b)}^2 \leq 2 a^2 + 2 b^2\), we can ``transfer'' the variance on \(\vx \) to the variance of \(\vx _*\). That is, \begin {align*} \mathbb {E} \norm {\rvvg \left (\vx \right )}_2^2 &= \mathbb {E} \norm {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right ) + \rvvg \left (\vx _*\right )}_2^2 \\ &\;\leq 2 \, \underbrace { \mathbb {E} \norm {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )}_2^2 }_{V_1} + 2 \, \underbrace { \mathbb {E} \norm {\rvvg \left (\vx _*\right )}_2^2 }_{V_2} \end {align*} \par The key is to bound \(V_1\). It is typical to do this using expected-smoothness-type assumptions such as the ER assumption. That is, \begin {align*} V_1 &= \mathbb {E} \norm {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )}_2^2 \\ &= \mathrm {tr}\V { \rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )} + \left ( \nabla F \left (\vx \right ) - \nabla F\left (\vx _*\right ) \right ), \shortintertext {from the \(L\)-smoothness of \(F\),} &\leq \mathrm {tr}\V { \rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )} + 2 L \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ), \shortintertext {and the ER condition,} &\leq 2 \mathcal {L} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ) + 2 L \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ) \\ &= 2 \left (L + \mathcal {L}\right ) \big ( F\left (\vx \right ) - F\left (\vx _*\right ) \big ). \end {align*} Finally, \(V_2\) immediately follows from the BV condition as \[ V_2 = \mathbb {E} \norm {\rvvg \left (\vx _*\right )}_2^2 \leq \sigma ^2. \]\end{proof}


==> main-pratendexpectedresidualwihtoutreplacement.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {thm:expected_residual_without_replacement} Let the objective function \(F\) satisfy \cref {assumption:components}, \(\pi \) be sampling \(b\) samples without replacement, and all elements of the solution set \(\vx _* \in \argmin _{\vx \in \mathcal {X}} F\left (\vx \right )\) be stationary points of \(F\). Then, the subsampling estimator \(\nabla f_{\rvB }\) satisfies the \(\mathrm {ER}\) condition as \begin {align*} &\mathrm {tr}\Vsub {\rvB \sim \pi }{ \nabla f_{\rvB }\left (\vx \right ) - \nabla f_{\rvB }\left (\vx _*\right ) } \\ &\qquad \leq 2 \frac {n - b}{b \left (n - 1\right )} L_{\mathrm {max}} \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ), \end {align*} where \(L_{\mathrm {max}} = \max \left \{L_1, \ldots , L_n\right \}\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}Consider that, for any random vector \(\rvvx \), \[ \mathrm {tr}\V {\rvvx ^2} \leq \mathbb {E}\norm {\rvvx }_2^2 \] holds. Also, sampling without replacement achieves \(b_{\mathrm {eff}} = \frac {(n-1) b}{n-b}\). Therefore, we have \begin {align*} &\mathrm {tr}\Vsub {\rvB \sim \pi }{ \nabla f_{\rvB }\left (\vx \right ) - \nabla f_{\rvB }\left (\vx _*\right ) } \\ &\;= \frac {n - b}{b \left (n - 1\right )} \mathrm {tr}\V { \nabla f_{i}\left (\vx \right ) - \nabla f_{i}\left (\vx _*\right ) } \\ &\;\leq \frac {n - b}{b \left (n - 1\right )} \left ( \frac {1}{n} \sum _{i=1}^n \norm { \nabla f_{i}\left (\vx \right ) - \nabla f_{i}\left (\vx _*\right ) }_2^2 \right ), \shortintertext {and from \cref {assumption:components},} &\;= \frac {n - b}{b \left (n - 1\right )} \left ( \frac {1}{n} \sum _{i=1}^n 2 L_i \mathrm {D}_{f_i}\left (\vx , \vx _* \right ) \right ). \shortintertext {Using the bound \(L_{\mathrm {max}} \geq L_i\) for all \(i = 1, \ldots , n\),} &\;\leq 2 L_{\mathrm {max}} \frac {n - b}{b \left (n - 1\right )} \left ( \frac {1}{n} \sum _{i=1}^n \mathrm {D}_{f_i}\left (\vx , \vx _* \right ) \right ), \shortintertext {applying \cref {thm:average_bregman},} &\;= 2 L_{\mathrm {max}} \frac {n - b}{b \left (n - 1\right )} \mathrm {D}_{F}\left (\vx , \vx _* \right ), \shortintertext {and since \(\vx _*\) is a stationary point of \(F\),} &\;= 2 \frac {n - b}{b \left (n - 1\right )} L_{\mathrm {max}} \left (F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \end {align*}\end{proof}


==> main-pratendexpectedsmoothnessreshuffling.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {thm:reshuffling_expected_smoothness} Let the objective function satisfy \cref {assumption:components}, \(B\) be any \(b\)-minibatch of indices such that \(B \subseteq \{1, \ldots , n\}\) and the component gradient estimators \(\rvvg _1, \ldots , \rvvg _n\) satisfy \cref {assumption:montecarlo_er} (\(\rm {A}^{\rm {CVX}}\)). Then, \(\rvvg _{B}\) is convex-smooth in expectation such that \begin {align*} \mathbb {E}_{\varphi }\norm {\rvvg _{B}\left (\vx \right ) - \rvvg _{B}\left (\vx _*\right )}_2^2 \leq 2 \left ( \mathcal {L}_{\rm {max}} + L_{\mathrm {max}} \right ) \mathrm {D}_{f_{B}} \left (\vx , \vx _*\right ), \end {align*} for any \(\vx \in \mathcal {X}\), where \begin {alignat*}{3} \vx _* &= \argmin _{\vx \in \mathcal {X}} F\left (\vx \right ), \\ \mathcal {L}_{\rm {max}} &= \max \left \{\mathcal {L}_{1}, \ldots , \mathcal {L}_{n} \right \}, \\ L_{\mathrm {max}} &= \max \left \{L_1, \ldots , L_n\right \}. \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvii}Notice that, for this Lemma, we do not assume that the minibatch \(B\) is a random variable. Therefore, the only randomness is the stochasticity of the component gradient estimators \(\rvvg _1, \ldots , \rvvg _n\). \par Now, from the property of the variance, we can decompose the expected squared norm as \begin {align*} &\mathbb {E} {\lVert \rvvg _B\left (\vx \right ) - \rvvg _B\left (\vx _*\right )\rVert }_2^2 \\ &\;= \underbrace { \mathrm {tr}\Vsub {\varphi }{ \rvvg _B\left (\vx \right ) - \rvvg _B\left (\vx _*\right ) } }_{V_{\rm {com}}} + \underbrace { {\lVert \nabla f_{B} \left (\vx \right ) - \nabla f_{B}\left (\vx _*\right ) \rVert }_2^2 }_{V_{\mathrm {sub}}}. \end {align*} \par First, the contribution of the variances of the component gradient estimators follows as \begin {align} V_{\rm {com}} &= \mathrm {tr}\Vsub {\varphi }{ \rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right ) } \nonumber \\ &= \mathrm {tr}\Vsub {\varphi }{ \frac {1}{b} \sum _{i \in B} \rvvg _{i}\left (\vx \right ) - \rvvg _{i}\left (\vx _*\right ) }, \nonumber \shortintertext {applying \cref {eq:varianceofsumeq2} of \cref {thm:varianceofsum},} &\leq \frac {1}{b} \sum _{i \in B} \mathrm {tr}\Vsub {\varphi }{ \rvvg _{i}\left (\vx \right ) - \rvvg _{i}\left (\vx _*\right ) }, \label {eq:loose_bound_for_reshuffling} \shortintertext {and then \cref {assumption:montecarlo_er} (\(\rm {A}^{\rm {CVX}}\)),} &\;\leq \frac {1}{b} \sum _{i \in B} 2 \mathcal {L}_{i} \, \mathrm {D}_{f_i}\left (\vx , \vx _*\right ). \nonumber \shortintertext {Now, since \(\mathcal {L}_{\mathrm {max}} \geq \mathcal {L}_i\) for all \(i= 1, \ldots , n\),} &\;\leq 2 \mathcal {L}_{\rm {max}} \frac {1}{b} \sum _{i \in B} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \nonumber \\ &\;= 2 \mathcal {L}_{\rm {max}} \mathrm {D}_{f_{B}}\left (\vx , \vx _*\right ). \nonumber \end {align} \par On the other hand, the squared error of subsampling (it is not the variance since we do not take expectation over the batches) follows as \begin {align*} V_{\mathrm {sub}} &= {\lVert \nabla f_{\rvB } \left (\vx \right ) - \nabla f_{\rvB }\left (\vx _*\right ) \rVert }_2^2 \\ &= \norm { \frac {1}{b} \sum _{i \in B} \nabla f_{i} \left (\vx \right ) - \nabla f_{i}\left (\vx _*\right ) }_2^2, \shortintertext {by Jensen's inequality,} &\leq \frac {1}{b} \sum _{i \in B} {\lVert \nabla f_{i} \left (\vx \right ) - \nabla f_{i}\left (\vx _*\right ) \rVert }_2^2, \shortintertext {from \cref {assumption:components},} &\leq \frac {1}{b} \sum _{i \in B} 2 L_{i} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \shortintertext {and since \(L_{\mathrm {max}} \geq L_i\) for all \(i= 1, \ldots , n\),} &\leq 2 L_{\mathrm {max}} \frac {1}{b} \sum _{i \in B} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \\ &= 2 L_{\mathrm {max}} \mathrm {D}_{f_B}\left (\vx , \vx _*\right ). \end {align*} Combining the bound on \(V_{\rm {com}}\) and \(V_{\rm {sub}}\) immediately yields the result.\end{proof}


==> main-pratendgeneralconditions.tex <==


\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxii}From \cref {thm:doubly_stochastic_variance}, we have \begin {align} &\mathrm {tr}\V {\rvvg _{\rvB }\left (\vx \right ) - \rvvg _{\rvB }\left (\vx _*\right )} \nonumber \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )} \right ) \nonumber \\ &\;\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )}} \right )}^2 \nonumber \\ &\;\qquad + \frac {1}{b_{\mathrm {eff}}} \mathrm {tr}\V {\nabla f_{\rvB }\left (\vx \right ) - \nabla F\left (\vx \right )}, \nonumber \shortintertext {where \cref {assumption:subsampling_er} yields} &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \underbrace { \left ( \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )} \right ) }_{\triangleq \mathrm {T_{\mathrm {var}}}} \nonumber \\ &\;\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) \underbrace { {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )}} \right )}^2 }_{\triangleq T_{\mathrm {cov}}} \nonumber \\ &\;\qquad + \frac {2 \mathcal {L}_{\mathrm {sub}} }{b_{\mathrm {eff}}} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ) \nonumber \\ &\;= \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) T_{\mathrm {var}} \nonumber + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) T_{\mathrm {cov}} \\ &\qquad + \frac {2 \mathcal {L}_{\mathrm {sub}} }{b_{\mathrm {eff}}} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \label {eq:master_equation_er} \end {align} \par \paragraph {Proof of \labelcref {thm:general_conditions_expected_residual1} with \((\rm {A}^{\rm {CVX}})\)} Since \cref {assumption:montecarlo_er}~\((\rm {A}^{\rm {CVX}})\) requires \(f_1, \ldots , f_n\) to be convex, \(F\) is also convex. Therefore, we can use the identity in \cref {thm:average_bregman} and \[ \mathrm {D}_{F}\left (\vx , \vx _*\right ) = F\left (\vx \right ) - F\left (\vx _*\right ). \] With that said, under \((\rm {A}^{\rm {CVX}})\), we have \begin {align} T_{\text {var}} &\leq \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )} \nonumber \\ &= \frac {1}{n} \sum ^n_{i=1} 2 \mathcal {L}_i \mathrm {D}_{f_i}\left (\vx , \vx _*\right ), \nonumber \shortintertext {applying \(\mathcal {L}_{\mathrm {max}} \geq \mathcal {L}_i\) for all \(i = 1, \ldots , n\),} &\leq 2 \mathcal {L}_{\mathrm {max}} \frac {1}{n} \sum ^n_{i=1} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \nonumber \shortintertext {and \cref {thm:average_bregman},} &= 2 \mathcal {L}_{\mathrm {max}} \mathrm {D}_{F}\left (\vx , \vx _*\right ). \label {eq:ercondition_item1_tvar} \end {align} \par For \(T_{\text {cov}}\), since \begin {align} T_{\text {cov}} &= {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )}} \right )}^2 \nonumber \shortintertext { is monotonic w.r.t. the variance, we can apply \((\rm {A}^{\rm {CVX}})\) as } &\leq \frac {2}{n^2} {\left ( \sum ^n_{i=1} \sqrt { \mathcal {L}_i \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) } \right )}^2. \nonumber \shortintertext {Now, applying the Cauchy-Schwarz inequality yields} &\leq \frac {2}{n^2} \left ( \sum ^n_{i=1} \mathcal {L}_i \right ) \left ( \sum ^n_{i=1} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \right ) \nonumber \\ &= 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathrm {D}_{f_i}\left (\vx , \vx _*\right ) \right ) \nonumber \shortintertext {and by \cref {thm:average_bregman},} &= 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \mathrm {D}_{F}\left (\vx , \vx _*\right ). \label {eq:ercondition_item1_tcov} \end {align} Plugging \cref {eq:ercondition_item1_tvar,eq:ercondition_item1_tcov} into \cref {eq:master_equation_er}, we have \begin {align*} &\mathrm {tr}\V {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )} \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) T_{\mathrm {var}} \nonumber + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) T_{\mathrm {cov}} \\ &\qquad + \frac {2 \mathcal {L}_{\mathrm {sub}} }{b_{\mathrm {eff}}} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ) \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) 2 \mathcal {L}_{\mathrm {max}} \mathrm {D}_{F}\left (\vx , \vx _*\right ) \\ &\;\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \mathrm {D}_{F}\left (\vx , \vx _*\right ) \\ &\;\qquad + \frac {1}{b_{\mathrm {eff}}} 2 \mathcal {L}_{\mathrm {sub}} \mathrm {D}_{F}\left (\vx , \vx _*\right ). \\ &= 2 \,\Bigg (\, \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \mathcal {L}_{\mathrm {max}} + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \\ &\qquad \qquad + \frac {1}{b_{\mathrm {eff}}} \mathcal {L}_{\mathrm {sub}} \,\Bigg )\, \mathrm {D}_{F}\left (\vx , \vx _*\right ) \\ &= 2 \,\Bigg (\, \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \mathcal {L}_{\mathrm {max}} + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \\ &\qquad \qquad + \frac {1}{b_{\mathrm {eff}}} \mathcal {L}_{\mathrm {sub}} \,\Bigg )\, \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \end {align*} \par \paragraph {Proof of \labelcref {thm:general_conditions_expected_residual1} with \((\rm {A}^{\rm {ITP}})\)} From \cref {assumption:montecarlo_er}~\((\rm {A}^{\rm {ITP}})\), we have \begin {align} T_{\text {var}} &= \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )} \nonumber \\ &\leq \frac {1}{n} \sum ^n_{i=1} 2 \mathcal {L}_i \left (f_i\left (\vx \right ) - f_i\left (\vx _*\right )\right ), \nonumber \shortintertext {applying \(\mathcal {L}_{\mathrm {max}} \geq \mathcal {L}_i\) for all \(i = 1, \ldots , n\),} &\leq 2 \mathcal {L}_{\mathrm {max}} \frac {1}{n} \sum ^n_{i=1} \left (f_i\left (\vx \right ) - f_i\left (\vx _*\right )\right ) \nonumber \\ &= 2 \mathcal {L}_{\mathrm {max}} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \label {eq:ercondition_item2_tvar} \end {align} \par Similarly, \begin {align} T_{\text {cov}} &= {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )}} \right )}^2, \nonumber \shortintertext {applying \((\rm {A}^{\rm {ITP}})\),} &\leq \frac {2}{n^2} {\left ( \sum ^n_{i=1} \sqrt { \mathcal {L}_i \left ( f_i\left (\vx \right ) - f_i\left (\vx _*\right ) \right ) } \right )}^2, \nonumber \shortintertext {and applying the Cauchy-Schwarz inequality,} &\leq \frac {2}{n^2} \left ( \sum ^n_{i=1} \mathcal {L}_i \right ) \left ( \sum ^n_{i=1} f_i\left (\vx \right ) - f_i\left (\vx _*\right ) \right ) \nonumber \\ &= 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \left ( \frac {1}{n} \sum ^n_{i=1} f_i\left (\vx \right ) - f_i\left (\vx _*\right ) \right ) \nonumber \\ &= 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \label {eq:ercondition_item2_tcov} \end {align} \par Plugging \cref {eq:ercondition_item2_tvar,eq:ercondition_item2_tcov} into \cref {eq:master_equation_er}, we have \begin {align*} &\mathrm {tr}\V {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )} \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) T_{\mathrm {var}} + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) T_{\mathrm {cov}} \\ &\qquad + \frac {2 \mathcal {L}_{\mathrm {sub}} }{b_{\mathrm {eff}}} \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ) \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) 2 \mathcal {L}_{\mathrm {max}} \left ( F\left (\vx \right ) F\left (\vx _*\right ) \right ) \\ &\;\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ) \\ &\;\qquad + \frac {1}{b_{\mathrm {eff}}} 2 \mathcal {L}_{\mathrm {sub}} \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ). \\ &= 2 \,\Bigg (\, \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \mathcal {L}_{\mathrm {max}} + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \\ &\qquad \qquad + \frac {1}{b_{\mathrm {eff}}} \mathcal {L}_{\mathrm {sub}} \,\Bigg )\, \left ( F\left (\vx \right ) - F\left (\vx _*\right )\right ). \end {align*} \par \paragraph {Proof of \labelcref {thm:general_conditions_expected_residual3}} From \cref {assumption:montecarlo_er} (B), we have \begin {align} T_{\text {var}} &= \frac {1}{n} \sum ^n_{i=1} \mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )} \nonumber \\ &\leq \frac {1}{n} \sum ^n_{i=1} 2 \mathcal {L}_i \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ) \nonumber \\ &= 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_{i} \right ) \left (F\left (\vx \right ) - F\left (\vx _*\right )\right ). \label {eq:ercondition_item3_tvar} \end {align} \par And, \begin {align} T_{\text {cov}} &= {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathrm {tr}\V {\rvvg _i\left (\vx \right ) - \rvvg _i\left (\vx _*\right )}} \right )}^2 \nonumber \\ &\leq \frac {2}{n^2} {\left ( \sum ^n_{i=1} \sqrt { \mathcal {L}_i \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ) } \right )}^2 \nonumber \\ &= 2 {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt { \mathcal {L}_i } \right )}^2 \left ( F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \label {eq:ercondition_item3_tcov} \end {align} \par Plugging \cref {eq:ercondition_item3_tcov,eq:ercondition_item3_tvar} into \cref {eq:master_equation_er}, we have \begin {align*} &\mathrm {tr}\V {\rvvg \left (\vx \right ) - \rvvg \left (\vx _*\right )} \\ &\;\leq \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) 2 \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \left (F\left (\vx \right ) - F\left (\vx _*\right ) \right ) \\ &\;\qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {2 \left ( \frac {1}{n} \sum ^n_{i=1} \sqrt { \mathcal {L}_i } \right )}^2 \left (F\left (\vx \right ) - F\left (\vx _*\right ) \right ) \\ &\;\qquad + \frac {1}{b_{\mathrm {eff}}} 2 \mathcal {L}_{\mathrm {sub}} \left (F\left (\vx \right ) - F\left (\vx _*\right ) \right ), \\ &\;= 2 \, \Bigg ( \left ( \frac {\rho }{b_{\mathrm {eff}}} + \frac {1 - \rho }{b} \right ) \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) \\ &\quad \qquad + \rho \left (1 - \frac {1}{b_{\mathrm {eff}}}\right ) {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt { \mathcal {L}_i } \right )}^2 \\ &\quad \qquad + \frac {1}{b_{\mathrm {eff}}} \mathcal {L}_{\mathrm {sub}} \Bigg ) \, \left (F\left (\vx \right ) - F\left (\vx _*\right ) \right ). \end {align*} \par \end{proof}


==> main-pratendgeometriccomplexity.tex <==


\begin{restatable}[Lemma A.2; \citealp {garrigos_handbook_2023}]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {thm:geometric_complexity} For a recurrence relation given as \[ r_{T} \leq {\left (1 - \gamma \mu \right )}^{T} r_{0} + B \gamma , \] for some constant \(0 < \gamma < 1/C\), \[r_T \leq \epsilon \] can be guaranteed by setting \begin {align*} \gamma &= \min \left (\frac {\epsilon }{2 B}, \frac {1}{C} \right ) \text { and } \\ T &\geq \frac {1}{\mu } \max \left (2 B \, \frac {1}{\epsilon }, C\right ) \log \left (2 \frac {r_0}{\epsilon }\right ), \end {align*} where \(\mu , B > 0\) and \(0 < C < \mu \) are some finite constants.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvii}First, notice that the recurrence \[ r_{T} \leq \underbrace {{\left (1 - \gamma \mu \right )}^{T} r_{0}}_{\text {bias}} + \underbrace { B \gamma }_{\text {variance}} , \] is a sum of monotonically increasing (variance) and decreasing (bias) terms with respect to \(\gamma \). Therefore, the bound is minimized when both terms are equal. This implies that \(r_t \leq \epsilon \) can be achieved by solving for \[ {\left (1 - \gamma \mu \right )}^{T} r_{0} \leq \frac {\epsilon }{2} \quad \text {and}\quad B \gamma \leq \frac {\epsilon }{2} \] First, for the variance term, \begin {alignat*}{3} B \gamma &\leq \frac {\epsilon }{2} \quad \Leftrightarrow \quad \gamma \leq \frac {\epsilon }{2 B}. \end {alignat*} \par For the bias term, as long as \(\gamma < \frac {1}{\mu }\), \begin {alignat*}{3} & & {\left (1 - \gamma \mu \right )}^{T} r_{0} &\leq \frac {\epsilon }{2} \\ &\Leftrightarrow &\qquad T \log {\left (1 - \gamma \mu \right )} &\leq \log \frac {\epsilon }{2 r_{0}} \\ &\Leftrightarrow &\qquad T &\leq \frac {\log \frac {\epsilon }{2 r_{0}}}{\log {\left (1 - \gamma \mu \right )}} \\ &\Leftrightarrow &\qquad T &\geq \frac {\log \frac {2 r_{0}}{\epsilon }}{ \log {\left (1/\left (1 - \gamma \mu \right )\right )}} \end {alignat*} Furthermore, using the bound \(\log 1/x \geq 1 - x \) for \(0 < x < 1\), we can achieve the guarantee with \[ T \geq \frac {1}{\gamma \mu } \log \left ( \frac {2 r_{0}}{\epsilon } \right ). \] Therefore, \(1/\gamma \) determines the iteration complexity. Plugging in the minimum over the constraints on \(\gamma \) yields the iteration complexity.\end{proof}


==> main-pratendgeometriccomplexitysquared.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {thm:geometric_complexity_squared} For a recurrence relation given as \[ r_{T} \leq {\left (1 - \gamma \mu \right )}^{T} r_{0} + A \gamma ^{2} + B \gamma , \] for some constant \(0 < \gamma < 1/C\), \[r_T \leq \epsilon \] can be guaranteed by setting \begin {align*} \gamma &= \min \left (\frac {-B + \sqrt {B^2 + 2A\epsilon }}{2 A}, \frac {1}{C} \right ) \text { and } \\ T &\geq \frac {1}{\mu } \max \left ( 2 B \, \frac {1}{\epsilon } + \sqrt {2 A}\,\frac {1}{\sqrt {\epsilon }}, C \right ) \log \left (2 \frac {r_0}{\epsilon }\right ), \end {align*} where \(\mu , A, B > 0\) and \(0 < C < \mu \) are some finite constants.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}This theorem is a generalization of Lemma A.2 by \citet {garrigos_handbook_2023}. First, notice that the recurrence \[ r_{T} \leq \underbrace {{\left (1 - \gamma \mu \right )}^{T} r_{0}}_{\text {bias}} + \underbrace { A \gamma ^{2} + B \gamma }_{\text {variance}} , \] is a sum of monotonically increasing (variance) and decreasing (bias) terms with respect to \(\gamma \). Therefore, the bound is minimized when both terms are equal. This implies that \(r_t \leq \epsilon \) can be achieved by solving for \[ {\left (1 - \gamma \mu \right )}^{T} r_{0} \leq \frac {\epsilon }{2} \quad \text {and}\quad A \gamma ^{2} + B \gamma \leq \frac {\epsilon }{2} \] First, for the variance term, \begin {alignat*}{3} & & A \gamma ^{2} + B \gamma &\leq \frac {\epsilon }{2} \\ &\Leftrightarrow &\qquad A \gamma ^{2} + B \gamma - \frac {\epsilon }{2} &\leq 0 \end {alignat*} The solution to this equation is given by the positive solution of the quadratic equation as \[ 0 < \gamma \leq \frac {- B + \sqrt { B^2 + 2 A \epsilon }}{2 A}. \] \par For the bias term, as long as \(\gamma < \frac {1}{\mu }\), the solution is identical to \cref {thm:geometric_complexity}. Therefore, \begin {equation} T \geq \frac {1}{\gamma \mu } \log \left ( \frac {2 r_{0}}{\epsilon } \right ) \label {eq:reshuffle_recurrence_t_lowerbound} \end {equation} can guarantee the bias term to be smaller than \(\nicefrac {\epsilon }{2}\), while \(1/\gamma \) determines the iteration complexity. Plugging in the minimum over the constraints on \(\gamma \), \begin {equation} \gamma = \min \left ( \frac {- B + \sqrt { B^2 + 2 A \epsilon }}{2 A}, \frac {1}{C}\right ) \label {eq:reshuffling_reccurrence_stepsize} \end {equation} yields the iteration complexity. \par Now, since the quadratic formula is not very interpretable, let us simplify the expression for \(1/\gamma \) using the bound \[ \frac {a}{2 \sqrt {b^2 + a}} \leq - b + \sqrt { b^2 + a}, \] which holds for any \(a,b > 0\) and is tight for \(\epsilon \to 0\). With our constants, this reads \begin {align*} \frac {A \epsilon }{\sqrt {B^2 + 2 A \epsilon }} \leq - B + \sqrt { B^2 + 2 A \epsilon }, \end {align*} and therefore \begin {align*} \frac {2 A}{- B + \sqrt { B^2 + 2 A \epsilon }} &\leq \frac {2 \sqrt {B^2 + 2 A \epsilon }}{\epsilon } \\ &\leq \frac {2 B + \sqrt {2 A \epsilon }}{\epsilon } \\ &= 2 B \frac {1}{\epsilon } + \sqrt {2 A} \frac {1}{\sqrt {\epsilon }}. \end {align*} Therefore, for the stepsize choice of \cref {eq:reshuffling_reccurrence_stepsize}, \[ \frac {1}{\gamma } \leq \min \left (2 B \frac {1}{\epsilon } + \sqrt {2 A} \frac {1}{\sqrt {\epsilon }}, \frac {1}{C}\right ). \] Plugging this into \cref {eq:reshuffle_recurrence_t_lowerbound} yields the statement.\end{proof}


==> main-pratendreshufflevariance.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexvi}\label{thm:prAtEndxvi}\label {thm:reshuffle_variance} For any \(b\)-minibatch reshuffling strategy, the squared error of the reference point of the Lyapunov function (\cref {eq:lyapunov_bias}) under reshuffling is bounded as \begin {align*} \mathbb {E} {\lVert \vx _{*}^{i} - \vx _*\rVert }_2^2 \leq \frac {\gamma ^2 n }{4 b^2} \, \tau ^2 \end {align*} for all \(i = 1, \ldots , p\), where \(\vx _* \in \argmin _{\vx \in \mathcal {X}} F\left (\vx \right )\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvi}The proof is a generalization of \citet [Proposition 1]{mishchenko_random_2020}, where we sample \(b\)-minibatches instead of single datapoints. Recall that \(\rvP \) denotes the (possibly random) partitioning of the \(n\) datapoints into \(b\)-minibatches \(\rvP _1, \ldots , \rvP _p\). From the definition of the squared error of the Lyapunov function in \cref {eq:lyapunov_bias}, we have \begin {align*} &\E { {\lVert \vx _{*}^{i} - \vx _*\rVert }_2^2 } \\ &\;= \E { \norm { \Pi _{\mathcal {X}}\left ( \vx _* - \sum _{k=0}^{i-1} \gamma \nabla f_{\rvP _i}\left (\vx _*\right ) \right ) - \Pi _{\mathcal {X}}\left (\vx _*\right ) }_2^2 }, \shortintertext {and since the projection onto a convex set under a Euclidean metric is non-expansive,} &\;\leq \E { \norm { \vx _* - \sum _{k=0}^{i-1} \gamma \nabla f_{\rvP _i}\left (\vx _*\right ) - \vx _* }_2^2 } \\ &\;= \E { \norm { \sum _{k=0}^{i-1} \gamma \nabla f_{\rvP _i}\left (\vx _*\right ) }_2^2 }, \shortintertext {introducing a factor of \(i\) in and out of the squared norm,} &\;= \frac {i^2}{2} \, \E { \norm { \frac {1}{i} \sum _{k=0}^{i-1} \gamma \nabla f_{\rvP _i}\left (\vx _*\right ) }_2^2 } \\ &\;= \frac {\gamma ^2 i^2}{2} \, \E { \norm { \frac {1}{i} \sum _{k=0}^{i-1} \nabla f_{\rvP _i}\left (\vx _*\right ) }_2^2 }. \end {align*} Now notice that \(\frac {1}{i} \sum ^{i-1}_{j=0} \nabla f_{\rvP _i} \left (\vx _*\right )\) is a sample average of \(i b\) samples drawn without replacement. Therefore, it is an unbiased estimate of \(\nabla F\left (\vx _*\right )\). This implies \begin {align*} \E { {\lVert \vx _{*}^{i} - \vx _*\rVert }_2^2 } &= \frac {\gamma ^2 i^2}{2} \, \E { \norm { \frac {1}{i} \sum _{k=0}^{i-1} \nabla f_{\rvP _i}\left (\vx _*\right ) }_2^2 } \\ &= \frac {\gamma ^2 i^2}{2} \, \mathrm {tr}\V { \frac {1}{i} \sum _{k=0}^{i-1} \nabla f_{\rvP _i}\left (\vx _*\right ) }, \shortintertext {and from \cref {thm:variancewithoutreplacement} with a sample size of \(ib\), } &= \frac {\gamma ^2 i^2}{2} \, \frac {n - ib}{\left (n-1\right ) ib} \frac {1}{n} \sum ^n_{i=1} \norm {\nabla f_{i}\left (\vx _*\right )}_2^2 \\ &= \frac {\gamma ^2 i \left (\frac {n}{b} - i\right )}{2 \left (n-1\right )} \tau ^2. \end {align*} Notice that this is a quadratic with respect to \(i\), where the maximum is obtained by \(i = \nicefrac {n}{2b}\). Then, \begin {align*} \E { {\lVert \vx _{*}^{i} - \vx _*\rVert }_2^2 } &\leq \frac {\gamma ^2 {\left (\frac {n}{2b}\right )}^2 }{2 \left (n-1\right )} \tau ^2 \\ &= \frac {\gamma ^2 n^2 }{8 b^2 \left (n-1\right )} \tau ^2, \shortintertext {and using the bound \(n/(n-1) \leq 2\) for all \(n \geq 2\),} &\leq \frac {\gamma ^2 n }{4 b^2} \, \tau ^2. \end {align*} \par \end{proof}


==> main-pratendstronglyconvexreshufflingsgdcomplexity.tex <==


\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxix}From the result of \cref {thm:strongly_convex_reshuffling_sgd_convergence}, we can invoke \cref {thm:geometric_complexity_squared} with \begin {alignat*}{3} A &= \frac {L_{\mathrm {max}} n}{4 b^2 \mu } \tau ^2,\quad \\ B &= \frac {2}{\mu }\left ( \frac {n-b}{(n-1) b} \left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}^2\right ) + \frac {n \left (b-1\right )}{\left (n-1\right ) b} {\left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2 \right ), \\ C &= \mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}}. \end {alignat*} Then, an \(\epsilon \) accurate solution in expectation can be obtained after \begin {align*} T &\geq \max \Bigg ( \underbrace {\frac {2 B}{\mu }}_{\triangleq C_1} \frac {1}{\epsilon } + \underbrace {\frac {\sqrt {2 A}}{\mu }}_{\triangleq C_2} \frac {1}{\sqrt {\epsilon }}, \; \frac {\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}}}{\mu } \Bigg ) \log \left (2 r_0^2 \frac {1}{\epsilon } \right ) \end {align*} iterations with a stepsize of \begin {align*} \gamma = \min \left ( \frac {- B + \sqrt {B^2 + 2 A \epsilon }}{2 A}, \frac {1}{C} \right ). \end {align*} To make the iteration complexity more precise, the terms \(C_1, C_2\) can be organized as \begin {align*} C_1 &= \frac {2 B}{\mu } = \frac {2}{\mu } \Bigg ( \, \frac {2}{\mu } \, \Bigg \{\, \frac {n-b}{(n-1) b} \left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}^2\right ) \\ &\qquad \qquad \qquad + \frac {n \left (b-1\right )}{\left (n-1\right ) b} {\left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2 \,\Bigg \} \,\Bigg ) \\ &= \frac {4}{\mu ^2} \Bigg ( \frac {n-b}{(n-1) b} \left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}^2\right ) + \frac {n \left (b-1\right )}{\left (n-1\right ) b} \, {\left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2 \Bigg ) \\ C_2 &= \frac {\sqrt {2 A}}{\mu } \\ &= \sqrt {2 \frac {L_{\mathrm {max}} n}{4 b^2 \mu } \tau ^2 } \frac {1}{\mu ^2} \\ &= \frac {\sqrt {L_{\mathrm {max}}} \, \tau \, \sqrt {n}}{\sqrt {2} b \mu ^{\nicefrac {3}{2}}} \\ &\leq \frac {\sqrt {L_{\mathrm {max}}}}{\mu ^{\nicefrac {3}{2}}} \frac { \sqrt {n}}{b} \, \tau . \end {align*} Applying the fact that \( (n-b)/n \leq (n-1)/n \leq 2 \) for all \( n \geq 2\) yields the simplified constants in the statement.\end{proof}


==> main-pratendstronglyconvexreshufflingsgdconvergence.tex <==


\begin{restatable}[]{theorem}{prAtEndRestatexviii}\label{thm:prAtEndxviii}\label {thm:strongly_convex_reshuffling_sgd_convergence} Let the objective \(F\) satisfy \cref {assumption:objective,assumption:components}, where, each component \(f_i\) is additionally \(\mu \)-strongly convex and \cref {assumption:montecarlo_er} (\(\rm {A}^{\rm {CVX}}\)), \labelcref {assumption:bounded_variance_both} hold. Then, the last iterate \(\vx _T\) of doubly SGD-RR with a stepsize satisfying \(\gamma < 1/\left (\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}}\right )\) guarantees \begin {align*} &\mathbb {E}{\lVert \vx _{K+1}^{0} - \vx _* \rVert }_2^2 \leq r^{K p} {\lVert \vx _1^{0} - \vx _* \rVert }_2^2 + C_{\mathrm {var}}^{\rm {sub}} \, \gamma ^2 + C_{\mathrm {var}}^{\rm {com}} \, \gamma \end {align*} where \(p = n/b\) is the number of epochs, \(\vx _* = \argmin _{\vx \in \mathcal {X}} F\left (\vx \right )\), \(r = 1 - \gamma \mu \) is the contraction coefficient, \begin {alignat*}{3} C_{\mathrm {var}}^{\rm {com}} &= { \frac {4}{\mu b} {\left ( \frac {1}{n} \sum ^n_{i=1} \sigma ^2_{i} \right )} + \frac {4}{\mu } \left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2, \text { and} \\ C_{\mathrm {var}}^{\rm {sub}} &= \frac {1}{4} \frac {L_{\mathrm {max}}}{\mu } \frac {n}{b^2} \left ( \frac {1}{n} \sum ^n_{i=1} \norm {\nabla f_i\left (\vx _*\right )}_2^2 \right ). \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxviii}The key element of the analysis of random reshuffling is that the Lyapunov function that achieves a fast convergence is \({\lVert \vx _k^{i+1} - \vx ^{i+1}_{*} \rVert }_2^2\) not \({\lVert \vx _{k}^{i+1} - \vx _* \rVert }_2^2\). This stems from the well-known fact that random reshuffling results in a conditionally biased gradient estimator. \par Recall that \(\rvP \) denotes the partitioning of the \(n\) datapoints into \(b\)-minibatches \(\rvP _1, \ldots , \rvP _p\). As usual, we first expand the Lyapunov function as \begin {align*} &{\lVert \vx ^{i+1}_k - \vx _*^{i+1}\rVert }_2^2 \\ &\;= {\lVert \Pi _{\mathcal {X}}(\vx ^{i}_k - \gamma \, \rvvg _{\rvP _i}(\vx ^i_k)) - \Pi _{\mathcal {X}}(\vx _*^i - \gamma \, \nabla f_{\rvP _i}\left (\vx _*\right ) ) \rVert }_2^2 \shortintertext {and since the projection onto a convex set under a Euclidean metric is non-expansive,} &\;\leq {\lVert (\vx ^{i}_k - \gamma \, \rvvg _{\rvP _i}(\vx ^i_k)) - (\vx _*^i - \gamma \, \nabla f_{\rvP _i}\left (\vx _*\right ) ) \rVert }_2^2 \\ &\;= {\lVert \vx ^{i}_k - \vx _*\rVert }_2^2 -2 \gamma \inner { \vx ^{i}_k - \vx _*^i \; }{ \rvvg _{\rvP _i}(\vx ^i_k) - \nabla f_{\rvP _i} \left (\vx _*\right ) } \\ &\qquad + \gamma ^2 {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \nabla f_{\rvP _i}\left (\vx _*\right )\rVert }_2^2. \end {align*} \par Taking expectation over the Monte Carlo noise conditional on the partitioning \(\rvP \), \begin {align*} &\mathbb {E}_{\varphi }{\lVert \vx ^{i+1}_k - \vx _*^{i+1}\rVert }_2^2 \\ &\;= {\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 -2 \gamma \inner { \vx ^{i}_k - \vx _*^i \; }{ \mathbb {E}_{\varphi }[\rvvg _{\rvP _i}(\vx ^i_k)] - \nabla f_{\rvP _i} \left (\vx _*\right ) } \\ &\qquad + \gamma ^2 \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \nabla f_{\rvP _i} \left (\vx _*\right ) \rVert } \\ &\;= {\lVert \vx ^{i}_k - \vx _*^i \rVert }_2^2 -2 \gamma \inner { \vx ^{i}_k - \vx _*^i \; }{ \nabla f_{\rvP _i}(\vx _k^i) - \nabla f_{\rvP _i}\left (\vx _*\right ) } \\ &\qquad + \gamma ^2 \, \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \nabla f_{\rvP _i} \left (\vx _*\right ) \rVert }_2^2. \end {align*} \par From the three-point identity, we can more precisely characterize the effect of the conditional bias such that \begin {align*} &\inner { \vx ^{i}_k - \vx _*^i \; }{ \nabla f_{\rvP _i}(\vx _k^i) - \nabla f_{\rvP _i}\left (\vx _*\right ) } \\ &= \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _k^i) + \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) - \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _*). \end {align*} \par For the gradient noise, \begin {align*} &\mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \nabla f_{\rvP _i} \left (\vx _*\right ) \rVert }_2^2 \\ &\;= \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \rvvg _{\rvP _i} \left (\vx _*\right ) + \rvvg _{\rvP _i}\left (\vx _*\right ) - \nabla f_{\rvP _i} \left (\vx _*\right ) \rVert }_2^2 \\ &\;\leq 2 \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \rvvg _{\rvP _i} \left (\vx _*\right ) \rVert }_2^2 + 2 \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}\left (\vx _*\right ) - \nabla f_{\rvP _i} \left (\vx _*\right ) \rVert }_2^2 \\ &\;= 2 \, \mathbb {E}_{\varphi } {\lVert \rvvg _{\rvP _i}(\vx ^i_k) - \rvvg _{\rvP _i} \left (\vx _*\right ) \rVert }_2^2 + 2 \, \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) }, \shortintertext {and from \cref {thm:reshuffling_expected_smoothness},} &\;\leq 4 \left ( \mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}} \right ) \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) + 2 \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } \end {align*} Notice the variance term \(\mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) }\). This quantifies the amount of deviation from the trajectory of singly stochastic random reshuffling. As such, it quantifies how slower we will be compared to its fast rate. \par Now, we will denote the \(\sigma \)-algebra formed by the randomness and the iterates up to the \(i\)th step of the \(k\)th epoch as \(\mathcal {F}_k^i\) such that \((\mathcal {F}_k^i)_{k \geq 1, i \geq 1}\) is a filtration. Then, \begin {align*} &\Esub {\rvveta _{k}^{i} \sim \varphi }{{\lVert \vx ^{i+1}_k - \vx _*^{i+1}\rVert }_2^2 \,\middle |\, \mathcal {F}_k^i} \\ &\leq {\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 \\ &\quad -2 \gamma \left ( \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _k^i) + \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) - \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _*) \right ) \\ &\quad + 4 \gamma ^2 \left (\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}}\right ) \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) \\ &\quad + 2 \gamma ^2 \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) }. \shortintertext {Now, the \(\mu \)-strong convexity of the component functions imply \(\mathrm {D}_{f_{\rvP _i}}\left (\vx _*^i, \vx _k^i\right ) \leq \frac {\mu }{2} {\lVert \vx _k^i - \vx _*^i \rVert }_2^2\). Therefore,} &\leq {\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 \\ &\quad - 2 \gamma \left ( \frac {\mu }{2} {\lVert \vx _k^i - \vx _*^i \rVert }_2^2 + \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) - \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _*) \right ) \\ &\quad + 4 \gamma ^2 \left ( \mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}} \right ) \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) \\ &\quad + 2 \gamma ^2 \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } , \shortintertext {and reorganizing the terms,} &= \left (1 - \gamma \mu \right ) {\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 \\ &\quad -2 \gamma \left (1 - 2 \gamma \left (\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}} \right )\right ) \mathrm {D}_{f_{\rvP _i}}(\vx _k^i, \vx _*) \\ &\quad + 2 \gamma \, \mathrm {D}_{f_{\rvP _i}}(\vx _*^i, \vx _*) \\ &\quad + \gamma ^2 2 \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) }. \end {align*} \par Taking full expectation, \begin {align} &\mathbb {E}{\lVert \vx ^{i+1}_k - \vx _*^{i+1}\rVert }_2^2 \nonumber \\ &\;\leq \left (1 - \gamma \mu \right ) \mathbb {E}{\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 \nonumber \\ &\quad - 2 \gamma \left (1 - 2 \gamma \left (\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}} \right )\right ) \E { \mathrm {D}_{f_{\rvP _i}}\left (\vx _k^n, \vx _*\right ) } \nonumber \\ &\quad + 2 \gamma \, \E { \mathrm {D}_{f_{\rvP _i}}\left (\vx _*^i, \vx _*\right )} \nonumber \\ &\quad + 2 \gamma ^2 \E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } }, \nonumber \shortintertext {and as long as \(\gamma < {1}/{\left ( 2 \left (\mathcal {L}_{\mathrm {max}} + L_{\mathrm {max}}\right ) \right )}\)} &\;\leq \left (1 - \gamma \mu \right ) \mathbb {E}{\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 + 2 \gamma \underbrace { \E { \mathrm {D}_{f_{\rvP _i}}\left (\vx _*^i, \vx _*\right )} }_{T_{\text {err}}} \nonumber \\ &\quad + 2 \gamma ^2 \underbrace { \E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } } }_{T_{\text {var}}} . \label {eq:reshuffling_convergence_main_bound} \end {align} \par \paragraph {Bounding \(T_{\mathrm {err}}\)} From the definition of the Bregman divergence and \(L\)-smoothness, for all \(j = 1, \ldots , n\), notice that we have \begin {align} \mathrm {D}_{f_j}\left ( \vy , \vx \right ) &= f_j\left (\vy \right ) - f_j\left (\vx \right ) - \inner {\nabla f_j\left (\vx \right )}{ \vy - \vx } \nonumber \\ &\leq \frac {L}{2} \norm {\vy - \vx }_2^2. \label {eq:bregman_smooth_upperbound} \end {align} for all \((\vx , \vx ') \in \mathcal {X}^2\). Given this, the Lyapunov error term \begin {align} \E { \mathrm {D}_{f_{\rvP _i}}\left (\vx _k^i, \vx _*\right ) } &= \E { \frac {1}{b} \sum _{j \in \rvP _i} \mathrm {D}_{f_{j}}\left (\vx _k^i, \vx _*\right ) } \nonumber \shortintertext {can be bounded using \(L\)-smoothness by \cref {eq:bregman_smooth_upperbound},} &\leq \E { \frac {1}{b} \sum _{j \in \rvP _i} \frac {L_{j}}{2} {\lVert \vx _k^i - \vx _*\rVert }_2^2 } \nonumber \shortintertext {and \(L_{\rm {max}} \geq L_i\) for all \(i = 1, \ldots , n\),} &\leq \frac {L_{\mathrm {max}}}{2} \E { \frac {1}{b} \sum _{j \in \rvP _i} {\lVert \vx _k^i - \vx _*\rVert }_2^2 } \nonumber \\ &= \frac {L_{\mathrm {max}}}{2} \mathbb {E} {\lVert \vx _k^i - \vx _*\rVert }_2^2. \label {eq:reshuffling_convergence_Terr} \end {align} \par The squared error \({\lVert \vx _k^i - \vx _*\rVert }_2^2\) is bounded in \cref {thm:reshuffle_variance} as \begin {equation} \mathbb {E} {\lVert \vx _k^i - \vx _*\rVert }_2^2 \leq \epsilon _{\mathrm {sfl}}^2 \triangleq \frac {\gamma ^2 n }{4 b^2} \, \tau ^2 < \infty . \label {eq:reshuffling_epsilon} \end {equation} \par \paragraph {Bounding \(T_{\mathrm {var}}\)} Now, let's take a look at the variance term. First, notice that, by the Law of Total Expectation, \begin {align*} \E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } } = \E { \E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } \mid \rvP } }. \end {align*} Here, \[ \E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } \mid \rvP } \] is the variance from selecting \(b\) samples without replacement. We can thus apply \cref {thm:expected_variance_lemma} with \(b_{\mathrm {eff}} = \frac {(n-1) b}{n-b}\) such that \begin {align} &\E { \mathrm {tr} \Vsub {\varphi }{ \rvvg _{\rvP _i}\left (\vx _*\right ) } \mid \rvP } \nonumber \\ &\;\leq \frac {n - b}{\left (n - 1\right ) b} \left (\frac {1}{n} \sum ^n_{j=1} \sigma ^2_{j}\right ) + \frac {n \left (b - 1\right )}{\left (n - 1\right ) b} {\left (\frac {1}{n} \sum ^n_{j=1} \sigma _{j}\right )}^2, \nonumber \shortintertext {which we will denote as} &\;= \sigma ^2 \label {eq:reshuffling_convergence_variance} \end {align} for clarity. Also, notice that \(\sigma ^2\) no longer depends on the partitioning. \par \paragraph {Per-step Recurrence Equation} Applying \cref {eq:reshuffling_convergence_Terr,eq:reshuffling_convergence_variance} to \cref {eq:reshuffling_convergence_main_bound}, we now have the recurrence equation \begin {align*} \mathbb {E}{\lVert \vx ^{i+1}_k - \vx _*^{i+1}\rVert }_2^2 &\leq \left (1 - \gamma \mu \right ) \mathbb {E}{\lVert \vx ^{i}_k - \vx _*^i\rVert }_2^2 \\ &\qquad + L_{\mathrm {max}} \epsilon _{\mathrm {sfl}}^2 \, \gamma + 2 \sigma ^2 \, \gamma ^2. \end {align*} \par Now that we have a contraction of the Lyapunov function \(\mathbb {E}{\lVert \vx _k^{i+1} - \vx _*^{i+1} \rVert }_2^2\), it remains to convert this that the Lyapunov function bounds our objective \(\mathbb {E}{\lVert \vx _k^{i+1} - \vx _* \rVert }_2^2\). This can be achieved by noticing that, at the end of each epoch, we have \(\vx _{k+1} - \vx _* = \vx ^{p}_{k} - \vx ^p_*\), and equivalently, we have \(\vx _k - \vx _* = \vx ^{0}_k - \vx ^{0}_*\) at the beginning of the epoch. The fact that the relationship with the original objective is only guaranteed at the endpoints (beginning and end of the epoch) is related to the fact that the bias of random reshuffling starts increasing at the beginning of the epoch and starts decreasing near the end. \par \paragraph {Per-Epoch Recurrence Equation} Nevertheless, this implies that by simply unrolling the recursion as in the analysis of regular SGD, we obtain a per-epoch contraction of \begin {align*} \mathbb {E}{\lVert \vx _{k+1}^0 - \vx _* \rVert }_2^2 &\leq {\left (1 - \gamma \mu \right )}^{p} \mathbb {E} {\lVert \vx _{k}^0 - \vx _* \rVert }_2^2 \\ &\quad + \left ( L_{\mathrm {max}} \epsilon ^2_{\mathrm {sfl}} \gamma + 2 \sigma ^2 \gamma ^2 \right ) \left (\sum ^{p-1}_{i=0} {\left (1 - \mu \gamma \right )}^{i} \right ). \end {align*} And after \(K\) epochs, \begin {align*} &\mathbb {E}{\lVert \vx _{K+1}^0 - \vx _* \rVert }_2^2 \leq {\left (1 - \gamma \mu \right )}^{p K} \mathbb {E} {\lVert \vx _{0}^0 - \vx _* \rVert }_2^2 \\ &+ \left ( L_{\mathrm {max}} \epsilon ^2_{\mathrm {sfl}} \gamma + 2 \sigma ^2 \gamma ^2 \right ) \left (\sum ^{p-1}_{i=0} {\left (1 - \mu \gamma \right )}^{i} \right ) \left (\sum ^{pK-1}_{j=0} {\left (1 - \mu \gamma \right )}^{p j} \right ). \end {align*} Note that \(T = pK\). \par As done by \citet {mishchenko_random_2020}, the product of sums can be bounded as \begin {align*} &\left (\sum ^{p-1}_{i=0} {\left (1 - \mu \gamma \right )}^{i} \right ) \left (\sum ^{T-1}_{j=0} {\left (1 - \mu \gamma \right )}^{p j} \right ) \\ &\;= \sum ^{p-1}_{i=0} \sum ^{T-1}_{j=0} {\left (1 - \mu \gamma \right )}^{i} {\left (1 - \mu \gamma \right )}^{p j} \\ &\;= \sum ^{p-1}_{i=0} \sum ^{T-1}_{j=0} {\left (1 - \mu \gamma \right )}^{i + pj} \\ &\;= \sum ^{Tp-1}_{i=0} {\left (1 - \mu \gamma \right )}^{i} \\ &\;\leq \sum ^{\infty }_{i=0} {\left (1 - \mu \gamma \right )}^{i} \\ &\;\leq \frac {1}{\gamma \mu }. \end {align*} Then, \begin {align*} &\mathbb {E}{\lVert \vx _{K+1}^0 - \vx _* \rVert }_2^2 \\ &\;\leq {\left (1 - \gamma \mu \right )}^{p K} \mathbb {E} {\lVert \vx _{0}^0 - \vx _* \rVert }_2^2 + \frac {1}{\gamma \mu } \left ( L_{\mathrm {max}} \epsilon ^2_{\mathrm {sfl}} \gamma + 2 \sigma ^2 \gamma ^2 \right ) \\ &= {\left (1 - \gamma \mu \right )}^{p K} \mathbb {E} {\lVert \vx _{0}^0 - \vx _* \rVert }_2^2 + \frac {\epsilon ^2_{\mathrm {sfl}} }{\mu } + \frac {2\sigma ^2}{\mu } \gamma . \end {align*} Plugging in the value of \(\epsilon _{\mathrm {sfl}}^2\) from \cref {eq:reshuffling_epsilon}, we have \begin {align*} \mathbb {E}{\lVert \vx _{K+1}^0 - \vx _* \rVert }_2^2 &\leq {\left (1 - \gamma \mu \right )}^{p K} \mathbb {E} {\lVert \vx _{0}^0 - \vx _* \rVert }_2^2 \\ &\qquad + \frac {L_{\mathrm {max}} n \sigma ^2_{\mathrm {sub}}}{4 b^2 \mu } \gamma ^2 + \frac {2\sigma ^2}{\mu } \gamma . \end {align*} This implies \begin {align*} &\mathbb {E}{\lVert \vx _{K+1}^{0} - \vx _* \rVert }_2^2 \leq r^{K n/b} {\lVert \vx _1^{0} - \vx _* \rVert }_2^2 + C_{\rm {var}}^{\mathrm {sub}} \, \gamma ^2 + C_{\rm {var}}^{\mathrm {com}} \, \gamma , \end {align*} where \(r = 1 - \gamma \mu \), \begin {alignat*}{3} C_{\rm {var}}^{\mathrm {sub}} &= \frac {1}{4} \frac {L_{\mathrm {max}}}{\mu } \frac {n}{b^2} \left ( \frac {1}{n} \sum ^n_{i=1} \norm {\nabla f_i\left (\vx _*\right )}_2^2 \right ), \text {and} \\ C_{\mathrm {var}}^{\rm {com}} &= { \frac {2}{\mu } \frac {n-b}{(n-1) b} {\left ( \frac {1}{n} \sum ^n_{i=1} \sigma ^2_{i} \right )} + \frac {2}{\mu } \frac {n \left (b-1\right )}{\left (n-1\right ) b} {\left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2 }. \end {alignat*} Applying the fact that \( (n-b)/n \leq (n-1)/n \leq 2 \) for all \( n \geq 2\) yields the simplified constants in the statement.\end{proof}


==> main-pratendstronglyconvexsgdcomplexity.tex <==


\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}We can apply \cref {thm:geometric_complexity} to the result of \cref {thm:strongly_convex_sgd_convergence} with the constants \[ r_0 = \norm {\vx _0 - \vx _*}_2^2, \quad B = \frac {2 \sigma ^2}{\mu }, \;\text {and}\;\; C = 2 \left ( \mathcal {L} + L \right ). \] Then, we can guarantee an \(\epsilon \)-accurate solution with the stepsize \[ \gamma = \min \left ( \frac {\epsilon \mu }{2 \sigma ^2}, \frac {1}{2 \left ( \mathcal {L} + L \right )} \right ) \] and a number of iterations of at least \begin {align*} T &\geq \frac {1}{\mu } \max \left ( \frac {2 \sigma ^2}{\mu }, 2 \left (\mathcal {L} + L\right ) \right ) \log \left (2 \norm {\vx _0 - \vx _*}_2^2 \frac {1}{\epsilon } \right ) \\ &= 2 \max \left ( \frac {\sigma ^2}{\mu ^2}, \frac {\mathcal {L} + L}{\mu } \right ) \log \left (2 \norm {\vx _0 - \vx _*}_2^2 \frac {1}{\epsilon } \right ). \end {align*} \par \end{proof}


==> main-pratendstronglyconvexsgdconvergence.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateiii}\label{thm:prAtEndiii}\label {thm:strongly_convex_sgd_convergence} Let the objective function \(F\) satisfy \cref {assumption:objective} and the gradient estimator \(\rvvg \) be unbiased and satisfy both \(\mathrm {ER}\left (\mathcal {L}\right )\) and \(\mathrm {BV}\left (\sigma ^2\right )\). Then, the last iterate of SGD guarantees {\setlength {\abovedisplayskip }{1ex} \setlength {\abovedisplayshortskip }{1ex} \setlength {\belowdisplayskip }{1ex} \setlength {\belowdisplayshortskip }{1ex} \[ \E { \norm {\vx _T - \vx ^*}_2^2 } \leq {\left (1 - \mu \gamma \right )}^{T} \norm {\vx _0 - \vx _*}_2^2 + \frac {2 \sigma ^2}{\mu } \gamma \] }where \(\vx _* = \argmin _{\vx \in \mathcal {X}} F\left (\vx \right )\) is the global optimum.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}Firstly, we have \begin {align*} &\norm {\vx _{t+1} - \vx _*}_2^2 \\ &\;= \norm {\Pi _{\mathcal {X}}\left ( \vx _{t} - \gamma \rvvg \left (\vx _t\right ) \right ) - \Pi \left (\vx _*\right )}_2^2, \shortintertext {and since the projection onto a convex set under a Euclidean metric is non-expansive,} &\;\leq \norm {\vx _{t} - \gamma \rvvg \left (\vx _t\right ) - \vx _*}_2^2 \\ &\;= \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \inner {\rvvg \left (\vx _t\right ) }{\vx _{t} - \vx _*} + \gamma ^2 \norm {\rvvg \left (\vx _t\right )}_2^2. \end {align*} Denoting the \(\sigma \)-algebra formed by the randomness and the iterates up to the \(t\)th iteration as \(\mathcal {F}_t\) such that \({(\mathcal {F}_t)}_{t \geq 1}\) forms a filtration, the conditional expectation is \begin {align*} &\E { \norm {\vx _{t+1} - \vx _*}_2^2 \mid \mathcal {F}_t } \\ &\;= \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \inner {\E { \rvvg \left (\vx _t\right ) \mid \mathcal {F}_t }}{\vx _{t} - \vx _*} \\ &\qquad + \gamma ^2 \E {\norm {\rvvg \left (\vx _t\right )}_2^2 \mid \mathcal {F}_t }. \\ &\;= \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \inner {\nabla F \left (\vx _t\right )}{\vx _{t} - \vx _*} \\ &\qquad + \gamma ^2 \E {\norm {\rvvg \left (\vx _t\right )}_2^2 \mid \mathcal {F}_t }, \shortintertext {applying the \(\mu \)-strong convexity of \(F\),} &\;\leq \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \left (F\left (\vx _t\right ) - F\left (\vx _*\right ) + \frac {\mu }{2} \norm {\vx _t - \vx _*}_2^2\right ) \\ &\qquad + \gamma ^2 \E {\norm {\rvvg \left (\vx _t\right )}_2^2 \mid \mathcal {F}_t } \\ &\;= \left (1 - \gamma \mu \right ) \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \left (F\left (\vx _t\right ) - F\left (\vx _*\right )\right ) \\ &\qquad + \gamma ^2 \E {\norm {\rvvg \left (\vx _t\right )}_2^2 \mid \mathcal {F}_t } \end {align*} \par From \cref {thm:expected_residual_gradient_variance_bound}, we have \begin {align*} \E {\norm {\rvvg \left (\vx _t\right )}_2^2 \mid \mathcal {F}_t } \leq \left (4 \left (\mathcal {L}+L\right ) \left (F\left (\vx _t\right ) - F\left (\vx _*\right ) \right ) + 2 \sigma ^2 \right ). \end {align*} Therefore, \begin {align*} &\E { \norm {\vx _{t+1} - \vx _*}_2^2 \mid \mathcal {F}_t } \\ &\leq \left (1 - \gamma \mu \right ) \norm {\vx _{t} - \vx _*}_2^2 - 2 \gamma \left (F\left (\vx _t\right ) - F\left (\vx _*\right )\right ) \\ &\quad + \gamma ^2 \left (4 \left (\mathcal {L}+L\right ) \left (F\left (\vx _t\right ) - F\left (\vx _*\right ) \right ) + 2 \sigma ^2 \right ) \\ &= \left (1 - \gamma \mu \right ) \norm {\vx _{t} - \vx _*}_2^2 \\ &\quad - 2 \gamma \left (1 - 2 \gamma \left (\mathcal {L} + L\right )\right ) \left (F\left (\vx _t\right ) - F\left (\vx _*\right )\right ) + 2 \gamma ^2 \sigma ^2, \shortintertext {and with a small-enough stepsize satisfying \(\gamma < \frac {1}{2 \left (\mathcal {L} + L\right )}\), we can guarantee a partial contraction as} &\leq \left (1 - \gamma \mu \right ) \norm {\vx _{t} - \vx _*}_2^2 + 2 \gamma ^2 \sigma ^2. \end {align*} Note that the coefficient \(1 - \gamma \mu \) is guaranteed to be strictly smaller than 1 since \(\mu \leq L\), which means that we indeed have a partial contraction. \par Now, taking full expectation, we have \[ \mathbb {E}\norm {\vx _{t+1} - \vx _*}_2^2 \leq \left (1 - \gamma \mu \right ) \mathbb {E}\norm {\vx _{t} - \vx _*}_2^2 + 2 \gamma ^2 \sigma ^2. \] Unrolling the recursion from \(0\) to \(T-1\), we have \begin {align*} \mathbb {E}\norm {\vx _{T} - \vx _*}_2^2 &\leq {\left (1 - \gamma \mu \right )}^T \mathbb {E}\norm {\vx _{0} - \vx _*}_2^2 \\ &\qquad + 2 \gamma ^2 \sigma ^2 \sum ^{T-1}_{t=0} {\left (1 - \gamma \mu \right )}^{t}. \\ &\leq {\left (1 - \gamma \mu \right )}^T \mathbb {E}\norm {\vx _{0} - \vx _*}_2^2 + \frac {2 \sigma ^2}{\mu } \gamma . \end {align*} where the last inequality follows from the asymptotic bound on geometric sums.\end{proof}


==> main-pratendstronglyconvexsgdsamplingwithoutreplacement.tex <==


\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxv}From \cref {assumption:components} and the assumption that \(\vx _*\) is a stationary point, \cref {thm:expected_residual_without_replacement} establishes that \(\nabla f_{\rvB }\) satisfies the \(\mathrm {ER}\left (\mathcal {L}_{\mathrm {sub}}\right )\) holds with \[ \mathcal {L}_{\mathrm {sub}} = \frac {n-b}{(n-1) b} L_{\mathrm {max}}. \] Therefore, \cref {assumption:subsampling_er} holds. Furthermore, since the component gradient estimators satisfy \cref {assumption:montecarlo_er} (B) and \cref {assumption:correlation} always hold with \(\rho = 1\), we can apply \cref {thm:general_conditions} which estblishes that \(\rvvg _{\rvB }\) satisfies \(\mathrm {ER}\left (\mathcal {L}\right )\) with \begin {align*} \mathcal {L} &= \frac {n-b}{(n-1) b} \left ( \frac {1}{n} \sum ^n_{i=1} \mathcal {L}_i \right ) + \frac {n (b-1)}{(n-1) b} {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\mathcal {L}_i} \right )}^2 \\ &\quad + \frac {n-b}{(n-1) b} L_{\mathrm {max}}. \end {align*} Furthermore, under \cref {assumption:bounded_variance_both}, \cref {thm:bounded_variance} shows that \(\mathrm {BV}\left (\sigma ^2\right )\) holds with \begin {align*} \sigma ^2 &= \frac {n-b}{(n-1) b} \left (\frac {1}{n} \sum ^n_{i=1} \sigma ^2_{i}\right ) + \frac {n (b-1)}{(n-1) b} {\left (\frac {1}{n} \sum ^n_{i=1} \sigma _{i}\right )}^2 \\ &\quad + \frac {n-b}{(n-1) b} \tau ^2. \end {align*} Since both \(\mathrm {ER}\left (\mathcal {L}\right )\) and \(\mathrm {BV}\left (\sigma ^2\right )\) hold and \(F\) satisfies \cref {assumption:objective}, we can now invoke \cref {thm:strongly_convex_sgd_complexity}, which guarantees that we can obtain an \(\epsilon \)-accurate solution after \[ T \geq 2 \max \Bigg ( \underbrace {\frac {\sigma ^2}{\mu ^2}}_{C_{\mathrm {var}}} \frac {1}{\epsilon }, \underbrace {\frac {\mathcal {L} + L}{\mu }}_{C_{\mathrm {bias}}} \Bigg ) \log \left (2 \norm {\vx _0 - \vx _*}_2^2 \frac {1}{\epsilon } \right ) \] iterations and fixed stepsize of \[ \gamma = \min \left ( \frac {\epsilon \mu }{2 \sigma ^2}, \frac {1}{2 \left (\mathcal {L} + L\right )} \right ). \] \par The constants in the lower bound on the number of required iterations can be made more precise as {\setlength {\abovedisplayskip }{1ex} \setlength {\abovedisplayshortskip }{1ex} \setlength {\belowdisplayskip }{1ex} \setlength {\belowdisplayshortskip }{1ex} \begin {align*} C_{\mathrm {var}} &= { \frac {n-b}{(n-1) b} \left ( {\frac {1}{n} \sum ^n_{i=1} \frac {\sigma _{i}^2}{\mu ^2} }\right ) } \\ &\quad + { \frac {n (b-1)}{(n-1) b} {\left ( \frac {1}{n} \sum ^n_{i=1} \frac {\sigma _{i}}{\mu } \right )}^2 + \frac {n-b}{(n-1)b} \frac {\tau ^2}{\mu ^2} } \\ C_{\mathrm {bias}} &= { \frac {n-b}{(n-1) b} \left ( {\frac {1}{n} \sum ^n_{i=1} \frac {\mathcal {L}_i}{\mu } }\right ) } \\ &\quad + { \frac {n (b-1)}{(n-1) b} {\left ( \frac {1}{n} \sum ^n_{i=1} \sqrt {\frac {\mathcal {L}_i}{\mu }} \right )}^2 + \frac {n-b}{(n-1) b} \frac {L}{\mu }. } \end {align*} Using the fact that \((n-b)/n \leq (n-1)/n \leq 2\) for all \(n \geq 2\) yields the simplified constants in the statement. }\end{proof}


==> main-pratendvarianceofsum.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevi}\label{thm:prAtEndvi}\label {thm:varianceofsum} Let \(\rvvx _1, \ldots , \rvvx _n\) be vector-variate random variables. Then, the variance of the sum is upper-bounded as \begin {align} \mathrm {tr}\V { \sum _{i=1}^n \rvvx _i } &\leq {\left ( {\textstyle \sum ^n_{i=1} \sqrt { \mathrm {tr}\V { \rvvx _i } } } \right )}^2 \label {eq:varianceofsumeq1} \\ &\leq n {\textstyle \sum ^n_{i=1} \mathrm {tr}\V { \rvvx _i }}. \label {eq:varianceofsumeq2} \end {align} The equality in \cref {eq:varianceofsumeq1} holds if and only if \(\rvvx _i\) and \(\rvvx _j\) are constant multiples such that there exists some \(\alpha _{ij} \geq 0\) such that {\setlength {\abovedisplayskip }{1ex} \setlength {\abovedisplayshortskip }{1ex} \setlength {\belowdisplayskip }{1ex} \setlength {\belowdisplayshortskip }{1ex} \[ \rvvx _i = \alpha _{ij} \rvvx _j \] }for all \(i, j\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvi}The variance of a sum is \begin {alignat*}{2} \mathrm {tr}\V { \sum _{i=1}^n \rvvx _i } = \sum _{i=1}^n \sum _{j=1}^n \mathrm {tr}\, \Cov {\rvvx _i, \rvvx _j}. \end {alignat*} From the Cauchy-Schwarz inequality for expectations, \begin {align*} \mathrm {tr}\, \Cov {\rvvx _i, \rvvx _j} &= \mathbb {E}{\left (\rvvx _i - \mathbb {E}\rvvx _i\right )}^{\top } {\left (\rvvx _j - \mathbb {E}\rvvx _j\right )} \\ &\leq \mathbb {E}\norm {\rvvx _i - \mathbb {E}\rvvx _i}_2 \mathbb {E}{\lVert \rvvx _j - \mathbb {E}\rvvx _j \rVert }_2 \\ &= \sqrt {\mathrm {tr}\V {\rvvx _i}} \sqrt {\mathrm {tr}\V {\rvvx _j}}. \end {align*} This implies \begin {alignat}{2} \mathrm {tr}\V { \sum _{i=1}^n \rvvx _i } &= \sum _{i=1}^n \sum _{j=1}^n \mathrm {tr}\,\Cov {\rvvx _i, \rvvx _j} \nonumber \\ &\leq \sum _{i=1}^n \sum _{j=1}^n \sqrt {\mathrm {tr}\V {\rvvx _i}} \sqrt {\mathrm {tr}\V {\rvvx _j}} \nonumber \\ &= {\left ( \sum _{i=1}^n \sqrt {\mathrm {tr}\V {\rvvx _i}} \right )}^2. \label {eq:sumofvariance_eq3} \end {alignat} The equality statement comes from the property of the Cauchy-Schwarz inequality. Lastly, \cref {eq:varianceofsumeq2} follows from additionally applying Jensen's inequality as \begin {alignat*}{2} {\left ( \sum _{i=1}^n \sqrt {\mathrm {tr}\V {\rvvx _i}} \right )}^2 &= n^2 {\left ( \frac {1}{n} \sum _{i=1}^n \sqrt {\mathrm {tr}\V {\rvvx _i}} \right )}^2 \\ &\leq n^2 \frac {1}{n} \sum _{i=1}^n {\left ( \sqrt {\mathrm {tr}\V {\rvvx _i}} \right )}^2 \\ &= n \sum _{i=1}^n \mathrm {tr}\V {\rvvx _i}. \end {alignat*} An equivalent proof strategy is to expand the quadratic in \cref {eq:sumofvariance_eq3} and apply the arithmetic mean-geometric mean inequality to the cross terms.\end{proof}


==> main-pratendvariancewithoutreplacement.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatev}\label{thm:prAtEndv}\label {thm:variancewithoutreplacement} Consider a finite population of \(n\) vector-variate random variables \(\vx _1, \ldots , \vx _n\). Then, the variance of the average of \(b\) samples chosen without replacement is \[ \mathrm {tr}\V { \frac {1}{b} \sum _{i=1}^b \rvvx _{\rvB _i} } = \frac {n - b}{b \left (n - 1\right )} \sigma ^2, \] where \(\rvB = \{\rvB _1, \ldots , \rvB _b\}\) is the collection of random indices of the samples and \(\sigma ^2\) is the variance of independently choosing a single sample.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndv}From the variance of the sum of random variables, we have \begin {alignat}{2} \mathrm {tr}\V { \sum _{i=1}^b \rvvx _{\rvB _i} } &= \sum _{i=1}^b \mathrm {tr}\V { \rvvx _{\rvB _i} } + \sum _{i=1}^b \sum _{i \neq j}^b \Cov {\rvvx _{\rvB _i}, \rvvx _{\rvB _j}}, \nonumber \shortintertext {and noticing that the covariance is independent of the index in the batch,} &= b \, \mathrm {tr}\V { \rvvx _{\rvB _i} } + b (b-1) C, \label {eq:sampling_wihout_replacement_eq1} \end {alignat} where \(C = \mathrm {Cov}\left (\rvvx _{\rvB _i}, \rvvx _{\rvB _j}\right )\). Using the fact that the variance is 0 for \(b = n\), we can solve for \(C\) such that \[ C = - \frac {1}{n-1}\, \mathrm {tr}\V { \rvvx _{\rvB _i} }, \] which is negative, and a negative correlation is always great. Plugging this expression to \cref {eq:sampling_wihout_replacement_eq1}, we have \begin {align*} \mathrm {tr}\V { \sum _{i=1}^b \rvvx _{\rvB _i} } &= b \, \mathrm {tr}\V { \rvvx _{\rvB _i} } - b (b-1) \frac {1}{n-1}\, \mathrm {tr}\V { \rvvx _{\rvB _i} }, \\ &= b \left (1 - \frac {b-1}{n-1} \right ) \mathrm {tr}\V { \rvvx _{\rvB _i} } \\ &= b\left (\frac {n - b}{n - 1}\right ) \mathrm {tr}\V { \rvvx _{\rvB _i} }. \end {align*} Dividing both sides by \(b^2\) yields the result.\end{proof}


==> section_kernel_regression.tex <==

\begin{align*}
  \minimize_{f \in \mathcal{H}}\; L\left(f\right) 
  &= \frac{1}{n} \sum^n_{i=1} \ell_i\left(f\left(\vx_i\right), y\right) + \frac{\lambda}{2} \norm{f}_{\mathcal{H}}^2
  \\
  &= \frac{1}{n} \sum^n_{i=1} r_i\left(f\right) + \frac{\lambda}{2} \norm{f}_{\mathcal{H}}^2,
\end{align*}
where we denoted the individual risk as
\[
  r_i\left(f\right) = \ell_i\left(f\left(\vx_i\right), y\right).
\]

The functional gradient is
\begin{align*}
  \left(\nabla_f r_i\right)\left(\cdot\right)
  &= \ell'\left(f\left(\vx_i\right), y_i\right) k\left(\vx, \cdot\right),
\shortintertext{and by Bochner's theorem,}  
  &= \ell'\left(f\left(\vx_i\right), y_i\right) \mathbb{E} \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right).
\end{align*}
Therefore, the Monte Carlo estimate of \(\nabla_f r_i\) is 
\[
  \rvvg_i\left(f\right) = \ell'\left(f\left(\vx_i\right), y_i\right) \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right),
\]
where \(\rvvz\) is the randomness.

In parameter space, this is implemented by
\[
  \Delta \alpha_i = 
\]

\newpage
\subsubsection{Preliminaries}

\begin{lemma}
    Let \(f : \mathcal{X} \to \mathbb{R} \in \mathcal{H}\) be a member of an RKHS \(\mathcal{H}\).
    Then,
    \[
      \abs{f\left(\vx\right)} 
      \leq 
      \sqrt{k\left(\vx, \vx\right)} \, \norm{ f }_{\mathcal{H}}
    \]
\end{lemma}
\begin{proof}
From the reproducing property of the RKHS, we have 
\[
  f\left(\vx\right) = \inner{f}{k\left(\vx, \cdot\right)}_{\mathcal{H}}.
\]
Therefore,
\begin{align*}
      \abs{f\left(\vx\right)} 
      &=
      \abs{\inner{f}{k\left(\vx, \cdot\right)}_{\mathcal{H}}},
\shortintertext{and by the Cauchy-Schwarz inequality,}
      &\leq
      \norm{k\left(\vx, \cdot\right)}_{\mathcal{H}} \norm{ f }_{\mathcal{H}}
      \\
      &=
      \sqrt{k\left(\vx, \vx\right)} \, \norm{ f }_{\mathcal{H}}.
\end{align*}
\end{proof}

\begin{assumption}
    The kernel function is bounded as
    \[
      k\left(\cdot, \cdot\right) \leq K < \infty.
    \]
\end{assumption}

\begin{lemma}
  Let \(\ell\left(\widehat{y}, y_i\right)\) be \(L_i\)-smooth with respect to \(\widehat{y}\).
  Then, \(r_i = \ell\left(f(\vx_i), y_i\right)\) is smooth in the RKHS such that
  \[
    \norm{ \nabla r_i\left(f\right) - \nabla r_i\left(h\right) }_{\mathcal{H}}
    \leq
    L_i K^{\nicefrac{3}{2}}
    \norm{f - h}_{\mathcal{H}}
  \]
  for all \(f, h \in \mathcal{H}\).
\end{lemma}
\begin{proof}
   \begin{align*}
     &\norm{ \nabla r_i\left(f\right) - \nabla r_i\left(h\right) }_{\mathcal{H}}
     \\
     &\;=
     \norm{ \ell'\left(f\left(\vx_i\right), y_i\right) k\left(\vx_i, \cdot\right) - \ell'\left(h\left(\vx_i\right), y_i\right) k\left(\vx_i, \cdot\right) }_{\mathcal{H}}
     \\
     &\;=
     \norm{ \left( \ell'\left(f\left(\vx_i\right), y_i\right) - \ell'\left(h\left(\vx_i\right), y_i\right) \right) k\left(\vx_i, \cdot\right) }_{\mathcal{H}}
     \\
     &\;\leq
     K \abs{ \ell'\left(f\left(\vx_i\right), y_i\right) - \ell'\left(h\left(\vx_i\right), y_i\right) }
     \\
     &\;\leq
     L_i K \norm{ f\left(\vx_i\right) - h\left(\vx_i\right) }_{\mathcal{H}}
     \\
     &\;\leq
     L_i K^{\nicefrac{3}{2}} \, \norm{ f - h }_{\mathcal{H}}.
   \end{align*} 
\end{proof}

First, we assume the random features are almost surely bounded:
\begin{assumption}
    The random features \(\phi\) have bounded variation as
    \[
      \mathbb{E}\norm{
        \frac{\phi_{\rvvz}\left(\vx_i\right) \phi_{\rvvz}\left(\cdot\right)}{k\left(\vx_i, \cdot\right)}
      }_{\mathcal{H}}^2
      = V_i < \infty
    \]
    for all \(\vz \in \mathcal{Z}\) and all \(\vx \in \mathcal{X}\).
\end{assumption}
This condition is satisfied by many popular random features.
In particular, most random features corresponding to stationary kernels (shift-invariant), such as the radial basis function (RBF), Mat\'ern, Laplace, Cauchy, and 1-layer neural network kernels with bounded activation functions, satisfy this.

\begin{align*}
  \norm{\ell'\left(f\left(\vx\right), y\right) - \ell'\left(h\left(\vx\right), y\right) }_2
  &\leq
  L \norm{f\left(\vx\right) - h\left(\vx\right)}_2
  \\
  &\leq
  L \norm{f - h}_{\mathcal{H}}
\end{align*}

\begin{align*}
    &\mathbb{E}\norm{ \rvvg_i\left(f\right) - \rvvg_i\left(h\right) }_{\mathrm{L}_2\left(\rho\right)}^2
    \\
    &=
    \mathbb{E}{\lVert
      \ell'\left(f\left(\vx_i\right), y_i\right) \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
      }
      \\
      &\quad\qquad-
      \ell'\left(h\left(\vx_i\right), y_i\right) \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
    {\rVert}_{\mathrm{L}_2\left(\rho\right)}^2
    \\
    &=
    \mathbb{E}\norm{
      \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
      \left(
        \ell'\left(f\left(\vx_i\right), y_i\right) 
        -
        \ell'\left(h\left(\vx_i\right), y_i\right)
      \right)
    }_{\mathrm{L}_2\left(\rho\right)}^2
    \\
    &=
    \mathbb{E}\norm{
      \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
    }_{\infty}^2
    {\left(
      \ell'\left(f\left(\vx_i\right), y_i\right) 
      -
      \ell'\left(h\left(\vx_i\right), y_i\right)
    \right)}^2
    \\
    &=
    L_i^2 \,
    \mathbb{E}\norm{
      \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
    }_{\mathrm{L}_2\left(\rho\right)}^2
    {\left(
      f\left(\vx_i\right)
      -
      h\left(\vx_i\right)
    \right)}^2
    \\
    &=
    L_i^2 \,
    \mathbb{E}\norm{
      \phi_{\rvvz}\left(\vx\right) \phi_{\rvvz}\left(\cdot\right)
    }_{\mathrm{L}_2\left(\rho\right)}^2
    \norm{ f - h }_{\mathcal{H}}^2
\end{align*}


==> thm_convex_sgd_convergence.tex <==

\begin{theoremEnd}[category=convexsgdconvergence]{lemma}
Let \(F : \mathcal{X} \to \mathbb{R}\) be convex and \(L\)-smooth on a convex set \(\mathcal{X}\).
Also, the gradient estimator \(\rvvg \in \mathrm{ER}\left(\mathcal{L}, F, F\right)\, \cap \,\mathrm{BV}\left(\sigma^2, F, F\right)\).
Then, for any stepsize schedule \(0 < \gamma_1, \ldots, \gamma_T < \frac{1}{2 \mathcal{L} + L}\),
\begin{align*}
  \E{ F\left(\bar{\vx}_T\right) - \inf F }
  \leq
  \frac{
    \frac{1}{2} \norm{\vx_0 - \vx_* }_2^2
    +
    \sigma^2 \sum^{T-1}_{t=0} \gamma_t^2
  }{\sum_{t=0}^{T-1} \gamma_t \left(1 - \gamma_i \left(2 \mathcal{L} + L\right) \right) },
\end{align*}
where \(\vx_* \in \argmin_{\vx \in \mathcal{X}} F\left(\vx\right)\).
\end{theoremEnd}

\begin{theoremEnd}[category=convexsgdconvergence]{corollary}
  Let the assumptions hold.
  Then, SGD achieves \(\epsilon\)-,  with \(\gamma = \frac{1}{\nicefrac{2 \sigma^2}{\epsilon} + 2 \mathcal{L} + L}\)
  \[
      T 
      \geq 
      {\left( 2 \sigma^2 \frac{1}{\epsilon^2} + \left(4 \mathcal{L} + 2 L\right) \frac{1}{\epsilon}  + \frac{{\left(2 \mathcal{L} + L\right)}^2}{2 \sigma^2} \right)}
      \norm{\vx_0 - \vx_* }_2^2.
  \]
\end{theoremEnd}
\begin{proofEnd}
For some fixed stepsize \(\gamma < \frac{1}{2 \mathcal{L} + L}\), where \(\alpha < 1\),  we have
\begin{align*}
  &\E{ F\left(\bar{\vx}_T\right) - \inf F }
  \\
  &\;\leq
  \frac{1
    \frac{1}{2} \norm{\vx_0 - \vx_* }_2^2
    +
    T \sigma^2 \gamma^2
  }{
    T \gamma \left(1 - \gamma \left(2 \mathcal{L} + L\right) \right)
  }
  \\
  &\;=
  \frac{\norm{\vx_0 - \vx_* }_2^2}{2 \gamma \left(1 - \gamma \left(2 \mathcal{L} + L\right) \right) }  \frac{1}{T} 
  +
  \frac{\sigma^2 \gamma}{1 - \gamma \left(2 \mathcal{L} + L\right)}.
\end{align*}

Since both terms are monotonic with respect to \(\gamma\), the optimum is achieved when both
\begin{align*}
  \frac{\norm{\vx_0 - \vx_* }_2^2}{2 \gamma \left(1 - \gamma \left(2 \mathcal{L} + L\right) \right) }  \frac{1}{T} 
  &\leq
  \frac{\epsilon}{2}
  \\
  \frac{\sigma^2 \gamma}{1 - \gamma \left(2 \mathcal{L} + L\right)}
  &\leq
  \frac{\epsilon}{2}
\end{align*}
hold.

First, the statistical term determines the largest stepsize we can choose such that
\begin{alignat*}{3}
  \frac{\sigma^2 \gamma}{1 - \gamma \left(2 \mathcal{L} + L\right)} \leq \frac{\epsilon}{2}
  \qquad\Leftrightarrow\qquad
  \gamma \leq \frac{1}{\nicefrac{2 \sigma^2}{\epsilon} + 2 \mathcal{L} + L }.
\end{alignat*}
This also automatically guarantees the stability constraint \(\gamma < \frac{1}{2 \mathcal{L} + L}\).
From now on, let us denote \(\widetilde{\mathcal{L}} = 2 \mathcal{L} + L\) for clarity.

For the optimization term, we have
\begin{alignat*}{2}
  & &
  \frac{1}{2 \gamma \left(1 - \gamma \widetilde{\mathcal{L}} \right) } \norm{\vx_0 - \vx_* }_2^2 \frac{1}{T} 
  \leq
  \frac{\epsilon}{2}
  \\
  &\Leftrightarrow& \qquad
  \frac{1}{\gamma \left(1 - \gamma \widetilde{\mathcal{L}} \right) } 
  \norm{\vx_0 - \vx_* }_2^2 \,
  \frac{1}{\epsilon}
  \leq
  T,
\end{alignat*}
Plugging in \(\gamma = \frac{1}{2 \sigma^2 / \epsilon + 2 \mathcal{L} + L} = \frac{1}{2 \sigma^2 / \epsilon + \widetilde{\mathcal{L}}}\),
\begin{alignat*}{2}
  T 
  &\geq 
  \frac{1}{\gamma \left(1 - \gamma \widetilde{\mathcal{L}} \right) } 
  \norm{\vx_0 - \vx_* }_2^2 \,
  \frac{1}{\epsilon}
  \\
  &=
  \frac{\nicefrac{2 \sigma^2}{\epsilon} + \widetilde{\mathcal{L}} }{ 1 - \frac{\widetilde{\mathcal{L}}}{\nicefrac{2 \sigma^2}{\epsilon} + \widetilde{\mathcal{L}}} } 
  \norm{\vx_0 - \vx_* }_2^2 \,
  \frac{1}{\epsilon}
  \\
  &=
  \frac{ {\left( \nicefrac{2 \sigma^2}{\epsilon} + \widetilde{\mathcal{L}} \right)}^2 }{ \nicefrac{2 \sigma^2}{\epsilon} } 
  \norm{\vx_0 - \vx_* }_2^2 \,
  \frac{1}{\epsilon}
  \\
  &=
  \frac{1}{2 \sigma^2}
  {\left( \frac{2 \sigma^2}{\epsilon} + \widetilde{\mathcal{L}} \right)}^2 
  \norm{\vx_0 - \vx_* }_2^2
  \\
  &=
  \frac{1}{2 \sigma^2}
  {\left( \frac{4 \sigma^4}{\epsilon^2} + 2 \frac{2 \sigma^2}{\epsilon} \widetilde{\mathcal{L}} + \widetilde{\mathcal{L}}^2 \right)}
  \norm{\vx_0 - \vx_* }_2^2
  \\
  &=
  {\left( 2 \sigma^2 \frac{1}{\epsilon^2} + 2 \widetilde{\mathcal{L}} \frac{1}{\epsilon}  + \frac{\widetilde{\mathcal{L}}^2}{2 \sigma^2} \right)}
  \norm{\vx_0 - \vx_* }_2^2.
\end{alignat*}
\end{proofEnd}

==> tikz_randnormal.tex <==
\newcount\gaussF
\edef\gaussR{0}
\edef\gaussA{0}

\makeatletter
\pgfmathdeclarefunction{gaussR}{0}{%
 \global\advance\gaussF by 1\relax
 \ifodd\gaussF
  \pgfmathrnd@%
  \ifdim\pgfmathresult pt=0.0pt\relax%
    \def\pgfmathresult{0.00001}%
  \fi
  \pgfmathln@{\pgfmathresult}%
  \pgfmathmultiply@{-2}{\pgfmathresult}%
  \pgfmathsqrt@{\pgfmathresult}%
  \global\let\gaussR=\pgfmathresult%radius
  \pgfmathrnd@%
  \pgfmathmultiply@{360}{\pgfmathresult}%
  \global\let\gaussA=\pgfmathresult%angle
  \pgfmathcos@{\pgfmathresult}%
  \pgfmathmultiply@{\pgfmathresult}{\gaussR}%
 \else
  \pgfmathsin@{\gaussA}%
  \pgfmathmultiply@{\gaussR}{\pgfmathresult}%
 \fi
}

\pgfmathdeclarefunction{invgauss}{2}{%
  \pgfmathln{#1}% <- might need parsing
  \pgfmathmultiply@{\pgfmathresult}{-2}%
  \pgfmathsqrt@{\pgfmathresult}%
  \let\@radius=\pgfmathresult%
  \pgfmathmultiply{6.28318531}{#2}% <- might need parsing
  \pgfmathdeg@{\pgfmathresult}%
  \pgfmathcos@{\pgfmathresult}%
  \pgfmathmultiply@{\pgfmathresult}{\@radius}%
}

\pgfmathdeclarefunction{randnormal}{0}{%
  \pgfmathrnd@
  \ifdim\pgfmathresult pt=0.0pt\relax%
    \def\pgfmathresult{0.00001}%
  \fi%
  \let\@tmp=\pgfmathresult%
  \pgfmathrnd@%
  \ifdim\pgfmathresult pt=0.0pt\relax%
    \def\pgfmathresult{0.00001}%
  \fi
  \pgfmathinvgauss@{\pgfmathresult}{\@tmp}%
}

==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

